Simultaneously Learning Stochastic and Adversarial Episodic MDPs with Known Transition

This work studies the problem of learning episodic Markov Decision Processes with known transition and bandit feedback. We develop the first algorithm with a ``best-of-both-worlds'' guarantee: it achieves $\mathcal{O}(log T)$ regret when the losses are stochastic, and simultaneously enjoys worst-case robustness with $\tilde{\mathcal{O}}(\sqrt{T})$ regret even when the losses are adversarial, where $T$ is the number of episodes. More generally, it achieves $\tilde{\mathcal{O}}(\sqrt{C})$ regret in an intermediate setting where the losses are corrupted by a total amount of $C$. Our algorithm is based on the Follow-the-Regularized-Leader method from Zimin and Neu (2013), with a novel hybrid regularizer inspired by recent works of Zimmert et al. (2019a, 2019b) for the special case of multi-armed bandits. Crucially, our regularizer admits a non-diagonal Hessian with a highly complicated inverse. Analyzing such a regularizer and deriving a particular self-bounding regret guarantee is our key technical contribution and might be of independent interest.

==> algorithm.tex <==
%!TEX root=main.tex
\section{Algorithm}
\label{sec:algoritm}
\begin{algorithm}[hb]
	\caption{Algorithm Pseudo Code}
	\label{alg:main_alg}
	\begin{algorithmic}
		\STATE {\bfseries Parameters:} state space $S$, action space $A$ and transition function $P$ (known to the learner)
		\STATE {\bfseries Initialize:} $\hatL_0 = (0,\ldots,0), \eta_t = 1/\sqrt{t}$ 
		\FOR{$t=1$ {\bfseries to} $T$}
		\STATE set $\psi_t(q) = -\frac{1}{\eta_t}\sum_{s,a} \rbr{\sqrt{ q(s,a) } + \sqrt{ q(s) - q(s,a) }} + C \sum_{s,a} \log\frac{1}{q(s,a)} $ 
		\STATE compute \[q_t = \argmin_{q\in\Omega} \inner{q, \hat{L}_{t-1}} + \psi_t(q)\] 
		\STATE where $\psi_t(q)$ is defined in Eq~\ref{eq:reguldef}
		\STATE observe $(s_0, a_0), \ldots, (s_{L-1}, a_{L-1})$ from interaction
		\STATE construct estimator $\hatl_t, \forall (s,a): \hatl_t(s,a) = \frac{\ell_t(s,a)}{q_t(s,a)}\Ind{s_{k(s)}=s,a_{k(s)}= a}$ 
		\STATE update $\hatL_t = \hatL_{t-1} + \hatl_t$
		\ENDFOR
	\end{algorithmic}
\end{algorithm}

The complete pseudocode of our algorithm is presented in Algorithm~\ref{alg:main_alg}. 
It is based on the general FTRL framework. In each episode $t$, the algorithm computes the regularized leader $q_t = \argmin_{q\in\Omega} \inner{q, \hat{L}_{t-1}} + \psi_t(q)$ where $\hat{L}_{t-1}=\sum_{\tau}^{t-1}\hat{\ell}_\tau$ is the cumulative estimate loss, and $\psi_t(q)$ is a hybrid regularizer $ \psi_t(q) = \eta_t^{-1} \phi_{main}(q) + \phi_{supp}(q)$ where  $\eta_t>0$ is a learning rate. 
Then the algorithm executes the induced policy $\pi_t = \pi^{q_t}$ associated with given transition function $P$. With the $L$ generated state-action pairs $(s_0, a_0), \ldots, (s_{L-1}, a_{L-1})$, the algorithm construct the loss estimator $\hatl_t(s,a) = \ell_t(s,a)\Ind{s_{k(s)}=s,a_{k(s)}= a} q(s,a)^{-1}$. 

The contribution of our work lies in the novel hybrid regularizer 
\begin{equation}
\label{eq:reguldef}
\begin{split}
\psi_t(q) & = \eta_t^{-1} \phi_{main}(q) + \phi_{supp}(q), \\
\phi_{main}(q) & = - \rbr{\sum_{s\in S\setminus\{s_L\},a\in A} \sqrt{ q(s,a) } + \alpha \sqrt{ q(s) - q(s,a) }}, \\
\phi_{supp}(q) & = C \sum_{s\in S\setminus\{s_L\},a\in A} \log\frac{1}{q(s,a)},  
\end{split}
\end{equation}
where we slightly abuse the notation to define 
\[
q(s) = \begin{cases} \sum_{s',a'} q(s',a')Pr(s|s',a'), &k(s) = 1, \ldots L - 1 \\ 1, &k(s) = 0\end{cases}
\]
and $C$ and $\alpha$ are two parameters with respect to the factors $|S|$, $|A|$ and $L$. 

==> main_proof.tex <==
%!TEX root=main.tex
\section{Main Proof}
\label{sec:proof}

\subsection{Follow the Regularized Leader}
\label{subsec:ftrl}

With a constant amount of log-barrier, the standard analysis of FTRLshows that the regret can be decomposed into several terms. 
\begin{lemma}
\label{lem:ftrl_main}
For $C=64L$ and learning rates $\cbr{\eta_t}_{t=1}^{T}$, our algorithm guarantees that $Reg_T(\pi)$, the regret with respect to referrer policy $\pi$, is upper-bounded by
\begin{equation}
\label{eq:ftrl_main}
\phi_{supp}(u) - \phi_{supp}(q_1) + \sum_{t=1}^{T}\rbr{\frac{1}{\eta_t} - \frac{1}{\eta_{t-1}}}\rbr{\phi_{main}(u) -\phi_{main}(q_t)} + 8\sum_{t=1}^{T}\E\sbr{\norm{\hatl_t}^2_{\nabla^{-2}\psi_t(q_t)}}
\end{equation}
\end{lemma}
where $u = q^{P,\pi}$ is the occupancy measure associated with transition function $P$ and referrer policy $\pi$, and $\eta_0$ is set to $+\infty$ by convention.

To prove Lemma~\ref{lem:ftrl_main}, we introduce the following notations
\begin{equation}
\begin{split}
F_{t} =  \inner{q_t, \widehat{L}_{t-1}}  + \phi_{t}(q) \;,& \;  G_{t} =  \inner{q_t, \widehat{L}_{t}}  + \phi_{t}(q) \\ 
q_{t} = \argmin_{q\in \Omega} F_t(q) \;,&\; \widetilde{q}_t = \argmin_{q \in \Omega} G_t(q) \\
\end{split}
\end{equation} 
With the help of these notations, the standard regret analysis of FTRL decompose the regret with referrer $u\in \Omega$ into \textit{penalty} and \text{stability} terms as follows 
\begin{equation}
\begin{split}
Reg_T(u) & = \E\sbr{\sum_{t=1}^{T} \inner{q_t - u, \hatl_t}}   \\
& = \underbrace{\E\sbr{\sum_{t=1}^{T} \cbr{\inner{q_t,\hatl_t} + F_t(q_t) - G_t(\tilde{q}_t)}}}_{stability}+ \underbrace{\E\sbr{\sum_{t=1}^{T} \cbr{ G_t(\tilde{q}_t) - F_t(q_t) - \inner{u, \hatl_t}}}}_{penalty}.
\end{split}
\end{equation}
In the rest of this sub-section, we will first prove tat the stability term is bounded by the sum of $\norm{\hatl_t}^2_{\nabla^{-2}\psi_t(q_t)}$, and second prove that the penalty term is controlled by the other terms in Eq.~\eqref{eq:ftrl_main}.

\begin{lemma}
	Given transition function $P$, for two occupancy measures $u$ and $v$, any $\lambda \in \rbr{0,1}$, the convex combination $\lambda u + (1-\lambda)v$ is a valid occupancy measure. 
	\label{lem:convex_combine}
\end{lemma}
\begin{proof}
	Fix $\lambda$, we verify the two basic properties in \cite{rosenberg19a} for $p=\lambda u + (1-\lambda)v$ is certainly in $\sbr{0,1}^{S\times A}$. We have 
	\begin{equation}
	\begin{split}
	p(s) & \triangleq \sum_{s',a'} Pr(s|s',a')p(s',a') \\
	& = \sum_{s',a'} Pr(s|s',a')\rbr{\lambda u(s',a') + (1-\lambda) v(s',a')} \\
	& = \lambda\sum_{s',a'}Pr(s|s',a')u(s',a')+ (1-\lambda)\sum_{s',a'}Pr(s|s',a')v(s',a') \\
	& = \lambda u(s) + (1-\lambda)v(s) \\
	& = \lambda \sum_{a} u(s,a) + (1-\lambda)\sum_{a} v(s,a) \\ 
	& = \sum_{a}  \rbr{\lambda u(s,a) + (1-\lambda) v(s,a)} \\ 
	& = \sum_{a} p(s,a).
	\end{split}
	\end{equation}
	And for state $s$ that $k(s) >0$, it holds that 
	\begin{equation}
	\begin{split}
	\sum_{s\in S_k}\sum_{a\in A}p(s,a) & = \lambda \sum_{s\in S_k}\sum_{a\in A}u(s,a) +  \rbr{1-\lambda} \sum_{s\in S_k}\sum_{a\in A}v(s,a)  \\
	& = \lambda + ( 1 - \lambda ) = 1  
	\end{split}
	\end{equation}
	which concludes that $p$ is a valid occupancy measure. 
\end{proof}

\begin{lemma}
	For occupancy measure $q$ and $p$ satisfying $\frac{1}{2}q(s,a) \leq p(s,a) \leq 2q(s,a)$ for all state-action pair $(s,a)$, it holds that $ \nabla^2 \psi(q) \geq \frac{1}{4} \nabla^2  \psi(p)$. 
	\label{lem:close_hessian}
\end{lemma}
\begin{proof} Let $A =  \nabla^2 \psi_t(p)$ and $B =  \nabla^2  \psi_t(q)$, for any vector $w$, we have 
	
	\begin{equation}
	\begin{split}
	w^\top B w & = \frac{1}{4\eta_t}\cbr{\frac{w(s,a)^2}{q(s,a)^{3/2}}
		+\frac{\alpha \rbr{\sum_{s',a'}P(s|s',a')w(s',a') - w(s,a)}^2}{(q(s)-q(s,a))^{3/2}}} + \frac{C}{4}\sum_{s,a} \frac{w(s,a)^2}{q(s,a)^2} 
	\end{split}
	\end{equation} 
	According to the fact that $q(s)-q(s,a) = \sum_{b\neq a}q(s,b)$ and $p(s)-p(s,a) = \sum_{b\neq a}p(s,b)$, we have $ \frac{1}{2}\rbr{q(s)-q(s,a)} \leq p(s)-p(s,a) \leq 2\rbr{q(s)-q(s,a)}$. Therefore, the following inequalities hold true 
	\begin{equation}
	\begin{split}
	w^\top B w&= \frac{1}{4\eta_t}\cbr{\frac{w(s,a)^2}{q(s,a)^{3/2}}
		+\frac{\alpha \rbr{\sum_{s',a'}P(s|s',a')w(s',a') - w(s,a)}^2}{(q(s)-q(s,a))^{3/2}}} + \frac{C}{4}\sum_{s,a} \frac{w(s,a)^2}{q(s,a)^2} \\ 
	& \geq \frac{1}{16\eta_t}\cbr{\frac{w(s,a)^2}{p(s,a)^{3/2}}
		+\frac{\alpha \rbr{\sum_{s',a'}P(s|s',a')w(s',a') - w(s,a)}^2}{(p(s)-p(s,a))^{3/2}}} + \frac{C}{16}\sum_{s,a} \frac{w(s,a)^2}{p(s,a)^2} \\
	& =\frac{1}{4} w^\top A w
	\end{split}
	\end{equation}
	where the second line follows from the fact $q(s,a)^{-3/2} \geq (2p(s,a))^{-3/2} \geq \frac{1}{4}p(s,a)^{-3/2}$ and the other similar facts. 
	which concludes that $\nabla^2 \psi_t(q)\geq \frac{1}{4}\nabla^2  \psi_t(p)$. 
\end{proof}

To bound the stability term, we first show that, when the coefficient $C$ is sufficiently large, $\tilde{q_t}$ is close to $q_t$ with respect to the norm over $\nabla^2\psi_t(q_t)$.

\begin{lemma}
	For $C = 64L$, we show that any $q'$ that satisfies $\norm{q'-q_t}_{\nabla^2\psi_t(q_t)} = 1 $ and $q' \in \Omega$, we have $G_t(q') \geq G_t(q_t)$, which indicates $\norm{\widetilde{q}_t-q_t}_{\nabla^2\psi_t(q_t)} \leq 1$.
	\label{lem:constrained_update}
\end{lemma}
\begin{proof}
	For simplicity, we denote the$H$ as the Hessian Matrix $\nabla^2 \psi_t(q_t)$, and $H_{supp}$ as the Hessian matrix of $\nabla^2 \psi_t(q_t)$. By the convexity of $\phi_{main}$, it holds that $H_{supp} \leq H$. Clearly, 
	$H_supp = diag\cbr{\frac{C}{q(s,a)^2}:(s,a)\in S\times A}$. 
	Fix the occupancy measure $q'$  that satisfies $\norm{q' - q_t}_{H} = 1$, we can show that 
	\begin{equation} 
	\begin{split}
	1 \geq \rbr{q' - q_t}^\top H_{supp} \rbr{q' - q_t} = C \sum_{s,a}\frac{\rbr{q'(s,a) - q_t(s,a)}^2 }{q_t(s,a)^2}.
	\end{split}
	\end{equation}
	Since $C\geq 9$, we have $\rbr{q'(s,a) - q_t(s,a)}^2 \leq \frac{q_t(s,a)^2}{C}  \leq  \rbr{\frac{q_t(s,a)}{3}}^2$, which indicates $\frac{1}{2} q_t(s,a) \leq  q'(s,a) \leq  2 q_t(s,a)$. 
	
	Fix $q'$, due to the first order optimality of $F_t(q_t)$, we have $\inner{\nabla F_t(q_t), q' - q_t} = 0$,. Therefore, we can expand $G_t(q')$ as 
	\begin{equation}
	\begin{split}
	G_t(q') & = G_t(q_t) + \nabla G_t(q_t)^\top(q'-q) + \frac{1}{2}(q'-q)^\top \nabla^2 \phi(\xi) (q'-q) \\
	& = G_t(q_t) + \nabla F_t(q_t)^\top(q'-q) + \hatl_t^\top(q'-q) + \frac{1}{2}(q'-q)^\top \nabla^2 \phi(\xi) (q'-q) \\
	& \geq G_t(q_t) - \norm{\hatl_t}_{H^{-1}} \norm{q'-q}_{H} + \frac{1}{2}\norm{q'-q}_{H}^2 \\
	& = G_t(q_t) - \norm{\hatl_t}_{H^{-1}}+ \frac{1}{2}\norm{q'-q}_{H}^2
	\end{split}
	\end{equation}
	where $\xi$ is a middle point in between $q_t$ and $q'$. 
	
	Because $\xi$ is a convex combination of $p'$ and $P_k$ and $P_k,p' \in \Omega$, we have $\xi \in \Omega$ by Lemma \ref{lem:convex_combine}. By Lemma \ref{lem:close_hessian}, it holds that 
	\begin{equation}
	\begin{split}
	& G_t(q_t) - \norm{\hatl_t}_{H^{-1}}+ \frac{1}{2}\norm{q'-q}_{H}^2 \\ \geq & G_t(q_t) - \norm{\hatl_t}_{H^{-1}}+ \frac{1}{8}\norm{q'-q}_{H}^2 \\ = & G_t(q_t) - \norm{\hatl_t}_{H^{-1}} + \frac{1}{8}
	\end{split}
	\label{eq:convex_eq}
	\end{equation}
	Then we consider bounding the term $\norm{\hatl_t}_{H^{-1}}$. By definition, the loss estimator satisfies that $ 0 \leq \ell_t \leq \frac{1}{q(s,a)}$. Due to the property of positive-definite matrix, we have $\nabla^{-2}\psi_t(q_t) \leq \nabla^{-2}\phi_{supp}(q_t) = H_{supp}^{-1}$ by the fact $\nabla^{2}\psi_t(q_t) > \nabla^{2}\psi_t(q_t)$. Therefore, we further have 
	\begin{equation}
	\begin{split}
	\norm{\hatl_t}^2_{H^{-1}} & =  \sum_{s,a}\sum_{s',a'}\cbr{\frac{\mathbb{I}(s,a)}{q(s,a)}\frac{\mathbb{I}(s',a')}{q(s',a')} H^{-1}\rbr{(s,a),(s',a')}} \\
	& \leq \sum_{s,a}\sum_{s',a'}\cbr{\frac{\mathbb{I}(s,a)}{q(s,a)}\frac{\mathbb{I}(s',a')}{q(s',a')} H_{supp}^{-1}\rbr{(s,a),(s',a')}} \\ 
	& = \sum_{s,a} \frac{\mathbb{I}(s,a)}{q(s,a)^2}H_{supp}^{-1}(s,a) \\
	& = \sum_{s,a} \frac{1}{C} \mathbb{I}\rbr{s,a} = \frac{L}{C} \leq \frac{1}{64}
	\end{split}
	\end{equation}
	Plugging it into Eq.~\eqref{eq:convex_eq}, we conclude that $\norm{\widetilde{q}_t - q_t}_{\nabla^2\psi_t(q_t)} \leq 1$, which indicates that $\frac{1}{2} q_t(s,a) \leq q_{t+1}(s,a) \leq 2 q_t(s,a)$ for all state-action pairs $(s,a)$. 
\end{proof}


\begin{lemma} For $C=64L$, it holds that 
	\begin{equation}
	\sum_{t=1}^{T} \cbr{\inner{q_t,\hatl_t} + F_t(q_t) - G_t(\tilde{q}_t)} \leq 8\sum_{t=1}^{T}\norm{\hatl_t}^2_{\nabla^{-2}\psi_t(q_t)}
	\end{equation}
	\label{lem:bound_stability}
\end{lemma}
\begin{proof} According to the optimality of $\tilde{q}_t$ and the convexity of $G_t$, the term $\inner{q_t,\hatl_t} + F_t(q_t) - G_t(\tilde{q}_t)$ can be upper-bounded as 
	\begin{equation}
	\begin{split}
	& \inner{q_t,\hatl_t} + F_t(q_t) - G_t(\tilde{q}_t) \\
	= & \inner{q_t, \hatl_t + \widehat{L}_{t-1}} + \psi_t(q_t) - G_t(\tilde{q}_t) \\ 
	= & G_t(q_t) - G_t(\tilde{q}_t) \\
	= & \inner{\nabla G_t(\tilde{q}_t),q _t - \tilde{q}_t } + \frac{1}{2}(q _t - \tilde{q}_t)^\top \nabla^2 \psi_t(\xi)  (q _t - \tilde{q}_t) \\
	\geq & \frac{1}{2} \norm{q _t - \tilde{q}_t}^2_{\nabla^2 \psi_t(\xi)}
	\end{split}.
	\end{equation}
	On the other hand, by the optimality of $q_t$ and the convexity of $F_t$, we have 
	\begin{equation}
	\begin{split}
	& \inner{q_t,\hatl_t} + F_t(q_t) - G_t(\tilde{q}_t) \\
	= & \inner{q_t - \tilde{q}_t ,\hatl_t} + F_t(q_t) - F_t(\tilde{q}_t) \\ 
	\leq & \inner{q_t - \tilde{q}_t ,\hatl_t}  \\ 
	\leq & \norm{q_t - \tilde{q}_t}_{\nabla^2 \psi_t(\xi)} \norm{\hatl_t}_{\nabla^{-2} \psi_t(\xi)}
	\end{split}
	\end{equation}
	By Lemma~\ref{lem:constrained_update}, we show that $\tilde{q}_t$ satisfies $\frac{1}{2} q_t(s,a) \leq \tilde{q}_t(s,a) \leq 2q(s,a)$ for all state-action pairs. Since $\xi$ is a middle point between $q_t$ and $\tilde{q}_t$, it satisfies $\frac{1}{2} q_t(s,a) \leq \xi(s,a) \leq 2q(s,a)$ for all state-action pairs as well. 
	According to Lemma~\ref{lem:close_hessian}  and, we finally get 
	\begin{equation}
	\inner{q_t,\hatl_t} + F_t(q_t) - G_t(\tilde{q}_t) \leq 2 \norm{\hatl_t}^2_{\nabla^{-2} \psi_t(\xi)} \leq 8  \norm{\hatl_t}^2_{\nabla^{-2} \psi_t(q_t)}
	\end{equation}
	which completes the proof.
\end{proof}


\begin{lemma}
	For any valid occupancy measure $u$, it holds that 
	\begin{equation}
	\begin{split}
	\sum_{t=1}^{T} &\cbr{ G_t(\tilde{q}_t) - F_t(q_t) - \inner{u, \hatl_t} }   \leq \phi_1(u)-\phi_1(q_1) + \sum_{t=2}^{T} \rbr{\frac{1}{\eta_t} - \frac{1}{\eta_{t-1}}  }\rbr{\phi_{main}(u) - \phi_{main}(q_t)} \\
	& = \phi_{supp}(u) - \phi_{supp}(q_1) + \sum_{t=1}^{T}\rbr{\frac{1}{\eta_t} - \frac{1}{\eta_{t-1}} }\rbr{\phi_{main}(u) - \phi_{main}(q_t)}.
	\end{split}
	\end{equation}
	\label{lem:bound_penalty}
\end{lemma}
\begin{proof} Due to the optimality of $G_t(\tilde{q_t})$, we have $G_t(\tilde{q_t}) \leq G_t(q_{t+1})$. Specially, we have $G_T(\tilde{q}_T) \leq G_T(u)$.  With the help fo these inequalities, we show that 
	\begin{equation}
	\begin{split}
	& \sum_{t=1}^{T} \cbr{ G_t(\tilde{q}_t) - F_t(q_t) - \inner{u, \hatl_t}} \\ 
	\leq & \sum_{t=1}^{T} \cbr{ G_t(q_{t+1}) - F_t(q_t) - \inner{u, \hatl_t}} \\ 
	= & - F_1(q_1) + \sum_{t=2}^{T} \rbr{ G_{t-1}(q_{t}) - F_t(q_t)} + G_T(u) - \inner{u, \hat{L}_T} \\
	= & - \phi_1(q_1) - \sum_{t=2}^{T}\rbr{\frac{1}{\eta_t} - \frac{1}{\eta_{t-1}} }\phi_{main}(q_t) + \psi_t(u) \\
	= & - \phi_{main}(q_1) -  \phi_{supp}(q_1) - \sum_{t=2}^{T}\rbr{\frac{1}{\eta_t} - \frac{1}{\eta_{t-1}} }\phi_{main}(q_t) + \frac{\phi_{main}(u)}{\eta_T} + \phi_{supp}(u) \\
	= & \phi_{supp}(u)  - \phi_{supp}(q_1) + \sum_{t=1}^{T} \rbr{\frac{1}{\eta_t} - \frac{1}{\eta_{t-1}} }\rbr{\phi_{main}(u) - \phi_{main}(q_t)} 
	\end{split}
	\end{equation} 
\end{proof}

Combining Lemma~\ref{lem:bound_stability} and Lemma~\ref{lem:bound_penalty} and  taking expectation proves Lemma~\ref{lem:ftrl_main}. In the rest part of this section, we will separately prove the following two key inequalities
 \begin{lemma} (Bound of Term $1$) For $C=64L$ and $\eta_t=\frac{\gamma}{\sqrt{t}}$, it holds that 
	\begin{equation}
	\begin{split}
	\sum_{t=1}^{T}&\rbr{\frac{1}{\eta_t} - \frac{1}{\eta_{t-1}}}\rbr{\phi_{main}(q^\star) -\phi_{main}(q_t)} \\
	 \leq & \sum_{t=1}^{T} \cbr{\frac{1+\alpha}{\gamma}\sum_{s\in S}\sum_{a\neq \pi^\star(a)}\sqrt{\frac{q_t(s,a)}{t}} + \frac{\rbr{1 + \alpha |A|}\sqrt{|S|L}}{\gamma}\sqrt{\sum_{s\in S}\sum_{a\neq \pi^\star(a)}\frac{q_t(s,a)}{t}}}
	\end{split}
	\end{equation}
	\label{lem:bound_term1}
\end{lemma}
where $|S|$ is the size of states and $|A|$ is the size of actions. 

 \begin{lemma} (Bound of Term $2$) By setting $C=64L$ and $\eta_t=\frac{\gamma}{\sqrt{t}}$, our algorithm guarantees that 
\begin{equation}
\sum_{t=1}^{T}\E\sbr{\norm{\hatl_t}^2_{\nabla^{-2} \psi_t(q_t)}} \leq 8eL^2\rbr{\sqrt{L} + \frac{1}{\alpha \cdot L} }\gamma \sum_{t=1}^{T}\sum_{s\in S}\sum_{a\neq \pi^\star(a)}\sqrt{\frac{q_t(s,a)}{t}}.
\end{equation}
\label{lem:bound_term2}
\end{lemma}
 
 \subsection{Proof of Lemma~\ref{lem:bound_term1}}

To help proving Lemma~\ref{lem:bound_term1}, we introduce following notations

 \begin{equation}
 \begin{split}
 g_t(s) = \sum_{a\in A}\rbr{\sqrt{q_t(s,a)} + \alpha \sqrt{q_t(s) - q_t(s,a)} }, &  
 h_t(s,a) = \rbr{\sqrt{\pi_t(s,a)} +  \alpha \sqrt{\sum_{a' \neq a} \pi_t(s,a')} } \\
 g^{\star}(s) = \sum_{a\in A}\rbr{\sqrt{q^\star(s,a)} +  \alpha \sqrt{q^\star(s) - q^\star(s,a)} }, &
 h^{\star}(s,a) = \rbr{\sqrt{\pi^\star(s,a)} + \alpha \sqrt{\sum_{a' \neq a} \pi^\star(s,a')} } \\
 \phi_{main}(q_t) = &-\sum_{s \in S} g_t(s) 
 \end{split}
 \end{equation}
 where $q_t$ is the selected occupancy measure of episode $t$, and $q^\star = q^{P,\pi^{\star}}$ is the occupancy measure associated with $P$ and optimal policy $\pi_t$. 
 
 
 	According to the property of occupancy measures, it holds that 
 	\[
 	\phi_{main}(q^\star) = -\sum_{s\in S}\sqrt{q^\star (s)}\sum_{a \in A} \rbr{ \sqrt{\pi^\star(s,a)} + \sqrt{\sum_{a' \neq a}\pi^\star(s,a')}  } = -\sum_{s\in S}\sqrt{q^\star (s)}\sum_{a \in A}h^\star(s,a).
 	\]
 	By the definition of the optimal policy, we have $\sum_{a}h^\star(s,a) = 1 + (|A|-1)\alpha$. 

 	We first show that the term $\phi_{main}(q^\star) - \phi_{main}(q_t)$ can be upper-bounded as 
 	\begin{lemma} It holds that 
 	\label{lem:phi_decompo_1}
 	\begin{equation}
 	\begin{split}
 	& \phi_{main}(q^\star) - \phi_{main}(q_t)\\ \leq & (1+\alpha) \sum_{s\in S\setminus\{s_L\}}\sum_{a \in A, a \neq \pi^{\star}(s)}\sqrt{q_t(s,a)}  + \rbr{ 1 + (|A|-1)\alpha}\sum_{s\in S}\rbr{\sqrt{q_t(s)} - \sqrt{q^\star(s)}} 
 	\end{split}
 	\end{equation}
 	\end{lemma}
 	

\begin{proof}
	First of all, $\phi_{main}(q^\star) - \phi_{main}(q_t)$ can be decomposed as 
	\begin{equation}
	\label{eq:wreg_phim_decomp}
	\begin{split}
	& \phi_{main}(q^\star) - \phi_{main}(q_t) \\ 
	= & \sum_{s\in S}\sqrt{q_t(s)} \sbr{\sum_{a\in A} h_t(s,a) -  \sum_{a\in A} h^\star(s,a)} + \sum_{s\in S}\sbr{\sqrt{q_t(s)} - \sqrt{q^\star(s)}} \sbr{\sum_{a\in A} h^\star(s,a)} \\
	= &\sum_{s\in S}\sqrt{q_t(s)} \sbr{\sum_{a\in A} h_t(s,a) -  \sum_{a\in A} h^\star(s,a)} 
	+ \rbr{1 + (|A|-1)\alpha}\sum_{s\in S}\rbr{\sqrt{q_t(s)} - \sqrt{q^\star(s)}} 
	\end{split}
	\end{equation}
	For the optimal action $a = \pi^\star(s)$, we have 
	\[
	\begin{split}
	h_t(s,a)  - h^\star(s,a) = & \sqrt{\pi_t(s,a)} + \alpha\sqrt{\sum_{a' \neq a} \pi_t(s,a')}  - 1 \\ 
	\leq & \alpha\sqrt{\sum_{a' \neq a} \pi_t(s,a')} \leq \alpha\sum_{a \neq \pi^\star(s)} \sqrt{\pi_t(s,a)} 
	\end{split}
	\]
	where the second line follows from the fact $\pi_t(s,a) \leq 1$. 
	
	For any other action $a$ that $a \neq \pi^\star(s)$, we have 
	\[
	h_t(s,a)  - h^\star(s,a) =  \sqrt{\pi_t(s,a)} + \alpha\sqrt{\sum_{a' \neq a} \pi_t(s,a')}  - \alpha \leq  \sqrt{\pi_t(s,a)}.
	\]
	Taking the summation, we have 
	\[
	\begin{split}
	& \sum_{a\in A} h_t(s,a) -  \sum_{a\in A} h^\star(s,a) \\ 
	\leq & h_t(s,\pi^\star(s))  - h^\star(s,\pi^\star(s)) + \sum_{a \neq \pi^{\star}(s) }\rbr{h_t(s,a)  - h^\star(s,a)} \\ 
	\leq & \alpha\sum_{a \neq \pi^\star(s)} \sqrt{\pi_t(s,a)}  + \sum_{a \neq \pi^\star(s)} \sqrt{\pi_t(s,a)} \\ 
	= & (1+\alpha) \sum_{a \neq \pi^\star(s)} \sqrt{\pi_t(s,a)} \\
	\end{split}
	\]
	which finishes the proof. 
\end{proof} 
      
    
    To help analyzing the term $\sqrt{q_t(s)} - \sqrt{q^\star(s)}$, we introduce the indicator $\mathbb{I}_{s} = \Ind{ q_t(s) \geq q^\star(s)}$. Therefore, we have that $\sqrt{q_t(s)} - \sqrt{q^\star(s)} \leq \sqrt{\mathbb{I}_{s} \rbr{q_t(s)-q^\star(s)}}$.  
  	\begin{lemma}
  	\label{lem:sqrt_diff}
  	For all state $s \in S\setminus \{s_L\}$, it holds that 
  	\begin{equation}
  	\sum_{s\in S}\sqrt{q_t(s)} - \sqrt{q^\star(s)} \leq \sum_{s\in S}\sqrt{\mathbb{I}_{s} \rbr{q_t(s)-q^\star(s)}} \leq \sqrt{|S|L} \sqrt{\sum_{s\in S\setminus \{s_L\}}\sum_{a \in A, a \neq \pi^{\star}(s)} q_t(s,a)}
  	\end{equation}
  	\end{lemma}
    \begin{proof}
    Fix the state $s$. When $k(s) = 0$, we can control the term by the fact $q_t(s_0) = q^\star(s) = 1$ . For $k(s)=k > 0 $, we plug Eq.~\eqref{eq:2} to 
    decompose this term as 
 	\begin{equation}
 	\begin{split}
 	q_t(s) - q^\star(s) & = \sum_{s' \in S_{k-1}}\sbr{q_t(s')\sum_{a\in A}\pi_t(s',a)P(s|s',a) - q^\star(s')\sum_{a\in A}\pi^\star(s',a)P(s|s',a)}.
 	\end{split}
 	\end{equation}
 	Then we discuss the bound of the term in the brackets into two cases. 
 	
 	For the $s'\in S_{k-1}$ satisfies $q_t(s') \leq q^\star(s')$, we have 
 	\begin{equation}
 	\begin{split}
 	& q_t(s')\sum_{a\in A}\pi_t(s',a)P(s|s',a) - q^\star(s')\sum_{a\in A}\pi^\star(s',a)P(s|s',a) \\
 	\leq & q_t(s')\sum_{a\in A}\pi_t(s',a)P(s|s',a) - q_t(s')\sum_{a\in A}\pi^\star(s',a)P(s|s',a) \\
 	= & q_t(s')\rbr{\sum_{a\in A}\pi_t(s',a)P(s|s',a) -P(s|s',\pi^\star(s'))} \\
 	= & q_t(s')\rbr{\sum_{a\neq \pi^\star(s')}\pi_t(s',a)\sbr{P(s|s',a) -P(s|s',\pi^\star(s'))}} \\
 	\leq & q_t(s')\sum_{a\neq \pi^\star(s')}\pi_t(s',a)Pr(s|s',a) \\ 
 	=& \sum_{a\neq \pi^\star(s')}q_t(s',a)Pr(s|s',a).
 	\end{split}
 	\label{eq:case1}
 	\end{equation}
 	For the other states that satisfies $q_t(s') \geq q^\star(s')$, we can further decompose the term as 
 	\begin{equation}
 	\label{eq:case2}
 	\begin{split}
 	& q_t(s')\sum_{a\in A}\pi_t(s',a)P(s|s',a) - q^\star(s')\sum_{a\in A}\pi^\star(s',a)P(s|s',a) \\
 	= & \rbr{q_t(s')-q^\star(s')}\sum_{a\in A}\pi_t(s',a)P(s|s',a) + q^\star(s')\sum_{a\in A}\rbr{\pi_t(s',a) - \pi^\star(s',a)}P(s|s',a) \\
 	\leq & \rbr{q_t(s')-q^\star(s')}\sum_{a\in A}\pi_t(s',a)P(s|s',a) + q^\star(s')\sum_{a\in A, a\neq \pi^\star(s)}\pi_t(s',a)Pr(s|s',a) \\
 	\leq & \rbr{q_t(s')-q^\star(s')}\sum_{a\in A}\pi_t(s',a)P(s|s',a) + q_t(s')\sum_{a\in A, a\neq \pi^\star(s)}\pi_t(s',a)Pr(s|s',a)
 	\end{split}
 	\end{equation}
 	where the third line follows the same technique in the previous case, and the last line follows the condition $q_t(s')\geq q^\star(s')$. 
 	
	By Eq.~\eqref{eq:case1} and Eq.~\eqref{eq:case2}, we show that the following inequality holds for all state $s\in S\setminus \{s_0,s_L\}$
	\begin{equation}
	\label{eq:twocases}
	\begin{split}
	\rbr{q_t(s) - q^\star(s)}\mathbb{I}_s \leq  & \sum_{s' \in S_{k-1}}q_t(s')\sum_{a\in A, a\neq \pi^\star(s)}\pi_t(s',a)Pr(s|s',a) \\ 
	 & +  \mathbb{I}_s\sum_{s' \in S_{k-1}}\Ind{q_t(s') \geq q^\star(s')}\rbr{q_t(s')-q^\star(s')}\sum_{a\in A}\pi_t(s',a)P(s|s',a) \\
	\leq & \sum_{s' \in S_{k-1}}\sum_{a\in A, a\neq \pi^\star(s)}q_t(s',a)Pr(s|s',a) \\
	 & + \sum_{s' \in S_{k-1}} \sbr{\rbr{q_t(s')-q^\star(s')}\mathbb{I}_{s'}} \cbr{ \sum_{a\in A}\pi_t(s',a)P(s|s',a) }
	\end{split}
	\end{equation}
	where the second line follows the non-negativity of the terms $\sbr{\rbr{q_t(s')-q^\star(s')}\mathbb{I}_{s'}}$ and the fact $0\leq \mathbb{I}_s \leq 1$. Besides, for $s_0$,  it's easy to verify that $q_t(s_0) - q^\star(s_0)=0$. 
	
	It's worth noting that the term $\sum_{a\in A}\pi_t(s',a)P(s|s',a) $ in curly brackets of Eq.~\eqref{eq:twocases}, is exactly the probability of reaching state $s$ from state $s'$. In other words, $\sum_{a\in A}\pi_t(s',a)P(s|s',a)$ equals to the following probability 
	\[
	\begin{split}
	&Pr\rbr{  \left. s_{k(s)} = s \right\lvert s_{k(s')} = s' , P , \pi_t    }  \triangleq p(s|s'), \\
	&Pr\rbr{  \left. s_{k(s)} = s \right\lvert s_{k(s')} = s' , a_{k(s')} = a, P , \pi_t    }  \triangleq p(s|s',a),\\
	\end{split}
	\]
	which we denoted such as $p(s|s')$ for all states $s,s'\in S$ that $k(s) = k(s') + 1$.  Clearly, such notation can generalize to state pairs that are not in two consecutive layers. Specifically, for every state $s,s'\in S_{k}$, we set $p(s|s') = \Ind{s = s'}$. For state $s$ and $s'$ that $k(s) = k > k(s') + 1  = k' + 1 $, we have 
	\[	
	\begin{split}
	p(s|s')  = &  Pr\rbr{  \left. s_{k} = s \right\lvert s_{k'} = s' , P , \pi_t    } \\
	= & \sum_{s_{m} \in S_{k-1} } Pr\rbr{  \left. s_{k} = s, s_{k-1} = s_{m} \right\lvert s_{k'} = s' , P , \pi_t  } \\
	= & \sum_{s_{m} \in S_{k-1} } Pr\rbr{  \left. s_{k} = s \right\lvert s_{k-1} = s_{m} , P , \pi_t  }  Pr\rbr{  \left. s_{k-1} = s_{m}  \right\lvert s_{k'} = s' , P , \pi_t  } \\
	= & \sum_{s_{m} \in S_{k-1} } p(s|s_{m}) p(s_{m}|s')
	\end{split} 
	\]
	where the second line uses the independence of visiting states in the same layer, and the third line follows from the Markov property. 
	Similarly, for states that $k(s) > k(s') + 1$,  it holds for $p(s|s',a)$ that 
	\[	
	\begin{split}
	p(s|s',a)  =  &  Pr\rbr{  \left. s_{k} = s \right\lvert s_{k'} = s', a_{k(s')} = a, P , \pi_t    } \\
	= & \sum_{s_{m} \in S_{k(s')+1} } Pr\rbr{  \left. s_{k} = s \right\lvert s_{k(s')} = s' ,a_{k(s')} = a, s_{k(s')+1} = s_{m} , P , \pi_t  } \\
	= &  \sum_{s_m\in S_{k(s')+1}} p(s|s_m)Pr(s_m|s',a).
	\end{split} 
	\]
	Specifically, for states $s,s'$ satisfying that $k(s)=k(s')+1$, we define $p(s|s',a) \triangleq Pr(s|s',a) =  \sum_{s_m\in S_{k(s')+1}} p(s|s_m)Pr(s_m|s',a)$. 
	
	With the help of such notions, we further simplify Eq.~\eqref{eq:twocases} as 
	\begin{equation}
	\label{eq:twocases_2}
	\begin{split}
	&  \sum_{s' \in S_{k-1}}q_t(s')\sum_{a\in A, a\neq \pi^\star(s)}\pi_t(s',a) + \sum_{s' \in S_{k-1}} \sbr{\rbr{q_t(s')-q^\star(s')} \mathbb{I}_{s'}} p(s|s')  \\ 
	\leq & \sum_{s' \in S_{k-1}}\sum_{a\in A, a\neq \pi^\star(s)}q_t(s',a)Pr(s|s',a) + \sum_{s_m \in S_{k-1}} \sum_{s' \in S_{k-2}} \sum_{a\in A, a\neq \pi^\star(s)}q_t(s',a)Pr(s_m|s',a)p(s|s_m) \\ 
	& +  \sum_{s'' \in S_{k-2}}\rbr{ \sum_{s' \in S_{k-1}}p(s|s')p(s'|s'')}  \sbr{\rbr{q_t(s'')-q^\star(s'')} \mathbb{I}_{s''}} \\ 
	= & \sum_{s' \in S_{k-1}}\sum_{a\in A, a\neq \pi^\star(s)}q_t(s',a)p(s|s',a) +\sum_{s' \in S_{k-2}} \sum_{a\in A, a\neq \pi^\star(s)}q_t(s',a)\rbr{\sum_{s_m \in S_{k-1}} Pr(s_m|s',a)p(s|s_m)} \\ 
	& +  \sum_{s'' \in S_{k-2}}\rbr{ \sum_{s' \in S_{k-1}}p(s|s')p(s'|s'')}  \sbr{\rbr{q_t(s'')-q^\star(s'')} \mathbb{I}_{s''}} \\ 
	= &  \sum_{s' \in S_{k-1}}\sum_{a\in A, a\neq \pi^\star(s)}q_t(s',a)Pr(s|s',a)+ \sum_{s' \in S_{k-2}} \sum_{a\in A, a\neq \pi^\star(s)}q_t(s',a)p(s|s',a) \\  
	& + \sum_{s'' \in S_{k-2}} p(s|s')\rbr{q_t(s'')-q^\star(s'')}  \\
	\leq & \sum_{k = 0}^{k(s)-1} \sum_{s' \in S_k} \sum_{a\in A, a\neq \pi^\star(s)}q(s',a)p(s|s',a) 
	\end{split}
	\end{equation}	
	where the second line follows the fact $\mathbb{I}_{s} \leq 1$ and $p(s|s) = 1$, the third line follows from the property of $p$, and the fourth line is done by recursively plugging the Eq.~\eqref{eq:twocases}.
	
	Taking the summation of all states, we have 
	\begin{equation}
	\begin{split}
	& \sum_{s\in S}\rbr{\sqrt{q_t(s)} - \sqrt{q^\star(s)}} \\ 
	\leq & \sum_{s\in S}\sqrt{\mathbb{I}_s\rbr{q_t(s) - q^\star(s)}} \\
	= &\sum_{s\in S} \sqrt{ \sum_{k = 0}^{l-1} \sum_{s' \in S_k}   \sum_{a\in A, a\neq \pi^\star(s)}q(s',a)p(s|s',a)}  \\
	\end{split}
	\end{equation}
	where the third line applies Eq.\eqref{eq:twocases_2}. Notice that, 
	\[
	\begin{split}
	 & \sum_{s\in S}  \sum_{k = 0}^{l-1} \sum_{s' \in S_k}   \sum_{a\in A, a\neq \pi^\star(s)}q(s',a)p(s|s',a)  \\
	= &  \sum_{k = 0}^{L-1} \sum_{s' \in S_k} q(s',a)\rbr{\sum_{l=k+1}^{L-1}p(s|s',a)} \\
	\leq & L \sum_{s' \in S} \sum_{s' \in S_k} q(s',a)
	\end{split}
	\]
	where the third line follows from the fact that $\sum_{s} p(s|s',a) \leq L$. 
	
	By H\"older's Inequality, we have 
	\[
	\begin{split}
	& \sum_{s\in S} \sqrt{ \sum_{k = 0}^{k(s)-1} \sum_{s' \in S_k}   \sum_{a\in A, a\neq \pi^\star(s)}q(s',a)p(s|s',a)\cdot 1}   \\
	\leq & \rbr{ \sum_{s\in S}  \sum_{k = 0}^{k(s)-1} \sum_{s' \in S_k}   \sum_{a\in A, a\neq \pi^\star(s)}q(s',a)p(s|s',a)}^{1/2} \rbr{\sum_{s\in S} 1}^{1/2}  \\
	= & \sqrt{|S|L} \sqrt{\sum_{s' \in S}  \sum_{a\in A, a\neq \pi^\star(s)} q_t(s',a)}.
	\end{split}	
	\]
	\end{proof}
 	
 	Combining Lemma~\ref{lem:sqrt_diff} and Lemma~\ref{lem:phi_decompo_1} yields that 
 	\[ 
 	\begin{split}
 	&\phi_{main}(q^\star) - \phi_{main}(q_t)\leq \\
 	&(1+\alpha)\sum_{s \in S\setminus \{s_L\} }\sum_{a\in A, a\neq \pi^\star(s)} \sqrt{q_t(s,a)}+ (1+\alpha|A|)\sqrt{|S|L} \sqrt{\sum_{s \in S\setminus \{s_L\} }\sum_{a\in A, a\neq \pi^\star(s)} q_t(s,a)}.
 	\end{split}
 	\]
 	Notice that $\frac{1}{\eta_t} - \frac{1}{\eta_{t-1}} \leq \frac{1}{\gamma \sqrt{t}}$, taking the summation from episode $1$ to $T$ finishes the proof of Lemma~\ref{lem:bound_term1}.

\subsection{Proof of Lemma~\ref{lem:bound_term2}}
Recall that $\nabla^2 \psi_t(q_t) \geq \eta_t^{-1} \nabla^2 \phi_{main}(q_t)$, which indicates $\nabla^{-2} \psi_t(q_t) \leq \eta_t \nabla^{-2} \phi_{main}(q_t)$. According to the property of positive definite matrices, the $\norm{\hatl_t}_{\nabla^{-2} \psi_t(q_t)}$ can be upper bounded by $\eta_t \norm{\hatl_t}_{\nabla^{-2} \phi_{main}(q_t)}$. For simplicity, in this section we drop the subscript $t$ of $q_t$, and prove the following key lemma. 

\begin{lemma}
\label{lem:bound_term2_main} For $\hatl_t$ such that $0\leq \hatl_t = \frac{\ell_t(s,a)\Ind{s_{k(s)}=s,a_{k(s)}=a}}{q(s,a)} \leq \frac{1}{q(s,a)}$ where $q\in\Omega$, it holds that 
\begin{equation}
\E\sbr{\norm{\hatl_t}_{\nabla^{-2}\phi_{main}(q)}^2} \leq 8eL^2\rbr{\sqrt{L}+\frac{1}{\alpha\cdot L}}\sum_{s \in S}\sum_{a\neq \pi^\star(s)}\sqrt{q(s,a)}
\end{equation}
\end{lemma}
By this lemma and the fact that $\eta_t = 1/\sqrt{t}$ we can directly prove the Lemma~\ref{lem:bound_term1}.


With the notations in Notation~\ref{para:matrix_notation}, we first carefully examine all second-order partial derivatives terms of $\phi_{main}$. 
The term $\sqrt{q(s,a)}$ in $\phi_{main}$ generates the second-order partial derivatives like:
\begin{equation}
\label{eq:sqrt_terms}
\frac{\partial^2 \phi_{main}}{\partial q(s,a)^2} \ni  \frac{1}{4}q(s,a)^{-3/2}
\end{equation}
On the other hand, the term $\alpha\sqrt{q(s)-q(s,a)}$ in $\phi_{main}$ generates the second-order partial derivatives like:
\begin{equation}
\label{eq:reverse_sqrt_terms}
\begin{split}
\frac{\partial^2 \phi_{main} }{\partial q(s',a')\partial q(s,a)}\ni -\frac{\alpha}{4}P(s|s',a')(q(s)-q(s,a))^{-3/2},\forall s'\in S_{k-1} \\
\frac{\partial^2 \phi_{main} }{\partial q(s',a')\partial q(s'',a'')}\ni \frac{\alpha}{4}P(s|s',a')P(s|s'',a'')(q(s)-q(s,a))^{-3/2},\forall s',s''\in S_{k-1} \\ 
\frac{\partial^2 \phi_{main} }{\partial q(s,a)^2}\ni \frac{\alpha}{4}(q(s)-q(s,a))^{-3/2}, \forall s'\in S_{k-1} \\ 
\end{split}
\end{equation}

Summarize the terms in Eq.~\eqref{eq:sqrt_terms} and Eq.~\eqref{eq:reverse_sqrt_terms}, the partial derivative over $q(s',a')$ and $q(s,a)$ can be represented as 
\begin{equation}
\begin{split}
\frac{\partial^2 \phi_{main}}{\partial q(s',a') \partial q(s,a)} & = -\frac{\alpha P(s|s',a')}{4}\rbr{q(s) - q(s,a)}^{-3/2},
s' \in S_{k-1}, s \in S_{k}, \\
\frac{\partial^2 \phi_{main}}{\partial q(s',a')  \partial q(s,a)}& = \frac{\alpha}{4}\sum_{s'',a''}P(s''|s,a)P(s''|s',a')(q(s'')-q(s'',a''))^{-3/2}, s,s'\in S_{k}  \\ 
\frac{\partial^2 \phi_{main}}{\partial q(s',a')  \partial q(s,a)}& = 0, (s,s'\notin S_{k}) \And (s\in S_{k} \And s'\notin S_{k-1}\bigcup S_{k+1}) \\
\frac{\partial^2 \phi_{main}}{ \partial q(s,a)^2}& = \frac{\alpha}{4} \sum_{s'\in S_{k+1},a'}{P(s'|s,a)^2}(q(s')-q(s',a'))^{-3/2} \\ &+ \frac{1}{4}(q(s,a))^{-3/2} + \frac{\alpha}{4}(q(s) - q(s,a))^{-3/2}
\end{split}
\label{eq:all_partial}
\end{equation}

To ensure that such regularizer is proper, we show that the Hessian matrix of $\phi_{main}$ is positive-definite for any $q \in \Omega$. 
\begin{lemma}
	$H = \nabla^2 \phi_{main}$ is positive-definite. 
	\label{lem:H_pos}
\end{lemma}
\begin{proof} For any vector $w$, we have 
	\begin{equation}
	\begin{split}
	w^\top H w = & \frac{1}{4}\sum_{s,a}q(s,a)^{-3/2}w(s,a)^2  \\
	+ & \frac{1}{4}\sum_{s,a}\alpha(q(s)-q(s,a))^{-3/2}\rbr{\sum_{s',a'}P(s|s',a')w(s',a') - w(s,a)}^2 \\
	\triangleq & \frac{1}{4}\sum_{s,a}\cbr{d(s,a)w(s,a)^2
		+ c(s,a)\rbr{\sum_{s',a'}P(s|s',a')w(s',a') - w(s,a)}^2}
	\end{split}
	\label{eq:Hessian_pos_def}
	\end{equation}where we denote $\alpha (q(s)-q(s,a))^{-3/2}$ by $c(s,a)$, and $q(s,a)^{-3/2}$ by $d(s,a)$ for simplicity. 
\end{proof}

\begin{lemma}
	For positive definite matrix $A\in \fR^{N\times N}$, it holds that $|A_{i,j}| \leq \frac{1}{2}\rbr{A_{i,i}+A_{j,j}} \forall i,j$.
\end{lemma}

Since Hessian matrix $H$ is positive-definite, there exists its inverse $H^{-1}$. which can be constructed layer by layer. For readability, we ignore the constant $\frac{1}{4}$ by considering the inverse matrix of $4H$. We will add this constant back in the proof of Lemma~\ref{lem:bound_term2_main}.

Let $M_k$ be the matrix of the partial derivatives terms that are only relevant with coefficients $d(s,a)$ or $c(s,a)$ for $(s,a) \in U_k$. For example, we have $M_0$ as follows:
\begin{equation}
M_0 = \begin{pmatrix}
c(s_0,a_1) + d(s_0,a_1) & 0 & 0 & \cdots & 0 \\
0 & c(s_0,a_2) + d(s_0,a_2) & 0 & \cdots & 0 \\
\vdots & \vdots & \vdots & \vdots & \vdots \\
0 & \cdots & \cdots & \cdots & c(s_0,a_{|A|}) + d(s_0,a_{|A|})
\end{pmatrix}
\end{equation}
where $A=\cbr{a_1,\ldots,a_{|A|}}$. Clearly, $M_0=diag\cbr{c(s,a)+d(s,a):s\in S_0,a\in A}$. 

For each layer $k = 0,\ldots,L-1$, we define the following matrices of $\fR^{U_k \times U_k}$
\begin{equation}
\begin{split}
I_k & = diag\cbr{1: (s,a) \in U_k}, \\
D_k & = diag\cbr{ d(s,a): (s,a) \in U_k } ,\\ 
C_k & = diag\cbr{ c(s,a): (s,a) \in U_k } .\\
\end{split}
\end{equation}
And for layer $k = 1,\ldots,L-1$, we define the following matrices for transition probabilities 
\begin{equation}
\begin{split}
P_k((s',a'),(s,a)) & = Pr(s|s',a'), \forall s\in S_{t-1},\forall s\in S_k ,  \\ 
\widetilde{P}_k((s',a'),(s,a)) & = \begin{cases}
Pr(s|s',a'),& \text{if } s' \in S_{t-1}\\
0,          & \text{if } s' \in S_{0:t-2}
\end{cases}.
\end{split}
\end{equation}
$I_k$ is the identity matrix of $\fR^{U_{k}\times U_{k}}$. $D_k \in \fR^{U_k\times U_k}$ can be regarded as the matrix of second-order partial derivatives in Eq.~\eqref{eq:sqrt_terms}. Similarly, $C_k\in \fR^{U_k\times U_k}$ represents the matrix of those in the third line of Eq.~\eqref{eq:reverse_sqrt_terms}. $P_k\in \fR^{U_{k-1}\times U_k}$ denotes the transition probabilities from previous layer to current layer. And its extension $\widetilde{P}_k$ is an matrix of $\fR^{U_{0:k-1}\times U_k}$ by adding preceding zeros to $P_k$.  We present a detailed Explanation in Figure~\ref{fig:matrix_def}.



	\begin{figure}
	\begin{center}
	\begin{tabular}{ |c|c|c|c| } 
		\hline
		\\[-1em]
		Name & Shape & Value \\ 
		\hline 
		\\[-1em]
		$I_k$ & $U_k \times U_k$ & $C_k((s,a),(s',a'))=\Ind{s=s',a=a'}$ \\ 
		\hline 
		\\[-1em]
		$C_k$ & $U_k \times U_k$ & $C_k((s,a),(s',a'))=c(s,a)\Ind{s=s',a=a'}$ \\ 
		\hline  
		\\[-1em]
		$D_k$ & $U_k \times U_k$ & $D_k((s,a),(s',a'))=d(s,a)\Ind{s=s',a=a'} $  \\
		\hline 
		\\[-1em]
		$P_k$ & $U_{k-1} \times U_k$ & $P_k((s,a),(s',a')) = Pr(s'|s,a)$  \\
		\hline
		\\[-1em]
		$\widetilde{P}_k$ & $U_{0:k-1} \times U_k$ & $\widetilde{P}_k((s,a)(s',a')) = \Ind{k(s) + 1 =k(s')}Pr(s'|s,a)$  \\ 
		\hline 
	\end{tabular}
	\end{center}
	\label{fig:matrix_def}
	\caption{Definitions of $I_k$, $C_k$, $D_k$, $P_k$ and $\widetilde{P}_k$ }
	\end{figure}


Then we show that the matrix $M_k$ can be represented by these matrices. 
\begin{lemma}With these notations, we have 
	$M_0 = C_0 + D_0$, and for $t>0$,
	\begin{equation}
	M_k = \begin{pmatrix}
	M_{k-1} + \widetilde{P}_k C_k \widetilde{P}_k^\top & -\widetilde{P}_k C_k \\
	-C_k \widetilde{P}_k^\top & C_k + D_k 
	\end{pmatrix}
	= \begin{pmatrix}
	M_{k-1}  &0 \\
	0 &  D_k 
	\end{pmatrix} +
	\begin{pmatrix}
	\widetilde{P}_k \\
	-I_t
	\end{pmatrix}
	C_k 
	\begin{pmatrix}
	\widetilde{P}_k^\top &
	-I_t
	\end{pmatrix}
	\end{equation}
	\label{lem:M_k_decomp}
\end{lemma}
\begin{proof}
	By definition, $M_0 = C_0 + D_0$. 
	For $M_k$, we verify each case according to Eq.~\eqref{eq:all_partial}.
	\begin{itemize}
		\item $(s,a),(s',a') \in U_{0:k-1}\times U_{0:k-1}$ and $(s,a),(s',a') \notin U_{k-1}\times U_{k-1} $: \\
		it holds that $M_{k-1}((s,a),(s',a')) = M_k((s,a),(s',a'))$. And since $\widetilde{P}_k((s,a),\cdot)=0$ or $\widetilde{P}_k((s',a'),\cdot)=0$, we have $\widetilde{P}_k C_k \widetilde{P}_k^\top((s,a),(s',a'))=0$.
		\item $(s,a)\in U_k, (s',a')\in U_{k-1}$: 
		\begin{equation*}
		\begin{split}
		M_k((s,a),(s',a')) & = -c(s,a)Pr(s|s',a') = -C_k((s,a),(s,a))P_k((s',a'),(s,a)) \\
		& = -\sum_{s'',a''\in U_k}C_k((s,a),(s'',a''))P_k^\top((s'',a''),(s',a')) \\ &= -\rbr{C_k P_k^\top}((s,a),(s',a'))  
		\end{split}
		\end{equation*} 
		By symmetry, the case $(s',a')\in U_k, (s',a')\in U_{t}$ is the same. 
		\item $(s,a),(s',a')\in U_k$:\\
		$M_k((s,a),(s',a')) = 0$ when $(s,a)\neq (s',a')$, and $M_k((s,a),(s,a)) = c(s,a) + d(s,a) = (C_k+D_k)((s,a),(s,a))$.
		\item $(s,a),(s',a')\in U_{k-1}$: \\
		\begin{equation*}
		\begin{split}
		& M_k((s,a),(s',a')) - M_0((s,a),(s',a')) = \sum_{s_1,a_1\in U_k}Pr(s_1|s,a)Pr(s_1|s',a')c(s'',a'')  \\  
		& = \sum_{s_1,a_1\in U_k}Pr(s_1|s,a)\rbr{\sum_{s_2,a_2\in U_k}Pr(s_2|s',a')C_k((s_1,a_1),(s_2,a_2))} \\
		& = \sum_{s_1,a_1\in U_k}P_k(s,a,s_1,a_1)\rbr{\sum_{s_2,a_2\in U_k}P_k^\top(s_2,a_2,s',a')C_k((s_1,a_1),(s_2,a_2))} \\
		& = \sum_{s_1,a_1\in U_k}P_k(s,a,s_1,a_1)\rbr{(C_k P_k^\top)(s_1,a_1,s',a')} = \rbr{P_k C_k P_k^\top} (s,a,s',a')
		\end{split}
		\end{equation*}
		Clearly, we have $\widetilde{P}_kC_k\widetilde{P}_k^\top(s,a,s',a') = P_k C_k P_k^\top (s,a,s',a')$. 
		
	\end{itemize}
	
	
\end{proof}

\begin{lemma}(Woodbury's Theorem) Assume $A$ and $C$ is invertible, we have 
	$$ (A + UCV) = A^{-1} - A^{-1}U\rbr{C^{-1} + VA^{-1}U}^{-1}VA^{-1}.$$
	\label{lem:woodbury}
\end{lemma}

By Lemma~\ref{lem:M_k_decomp} and ~\ref{lem:woodbury}, we have 
\begin{equation}
\begin{split}
M_k^{-1} &= \begin{pmatrix}M_{k-1}^{-1} & 0\\ 0 & D_k^{-1} \end{pmatrix} - \begin{pmatrix}M_{k-1}^{-1}P_k \\ -D_k^{-1} \end{pmatrix}
\rbr{ C_k^{-1} + D_k^{-1}+P_k^\top M^{-1}_{t-1}P_k}^{-1}  
\begin{pmatrix}P_k^\top M_{k-1}^{-1} & -D_k^{-1}\end{pmatrix}
\\& =\begin{pmatrix}
M_{k-1}^{-1} - M_{k-1}^{-1} P_k S_k P_k^\top  M_{k-1}^{-1} & M_{k-1}^{-1} P_k S_k D_k^{-1}\\
D_k^{-1} S_k P_k^\top M_{k-1}^{-1}  & D_k^{-1} - D_k^{-1} S_k D_k^{-1} 
\end{pmatrix}   
\end{split}
\label{eq:M_k_inv_decomp}
\end{equation}
where $S_k = ( C_k^{-1} + D_k^{-1} + P_k^\top M_{k-1}^{-1} P_k )^{-1}$. 

Let $N_0 = M_0^{-1}$ and $N_k = D_k^{-1} - D_k^{-1} S_k D_k^{-1}$. In other words, the $N_k$ is the right-bottom square matrix of the $M_k^{-1}$, the projection of $M_k^{-1}$ onto $U_k\times U_k$. 


\begin{lemma}
	For any vector $w_k\in \fR^{U_k}$, it holds that $$
	\begin{pmatrix}
	\mathbf{0}_{U_{0:k-1}}^\top,w_k^\top, \mathbf{0}_{U_{k+1:L-1}}^\top
	\end{pmatrix} (4H)^{-1} \begin{pmatrix}
	\mathbf{0}_{U_{0:k-1}} \\ w_k \\\mathbf{0}_{U_{k+1:L-1}}
	\end{pmatrix} \leq w_k^\top N_k w_k.$$
	\label{lem:N_over_H}
	where $\mathbf{0}_S\in \fR^S$ only contains zeros when $S = U_{0:k-1}$ or $S = U_{k+1:L-1} \triangleq U_{L-1} \setminus U_{t}$. 
\end{lemma}
\begin{proof} The matrices $M_k$ and $D_{t+1},\ldots,D_L$ can construct a positive definite block diagonal matrix $\widetilde{M}_k = diag\cbr{M_k,D_{t+1},\ldots,D_L} \leq 4H$, hence $\widetilde{M}_k^{-1}=diag\cbr{M_k^{-1},D_{t+1}^{-1},\ldots,D_L^{-1}} \geq (4H)^{-1}$. 
	
	Therefore, for the $w_k$ described in the lemma, we have  
	\begin{equation*}
	\begin{split}
	&
	\begin{pmatrix}
	\mathbf{0}_{U_{0:k-1}}^\top,w_k^\top, \mathbf{0}_{U_{k+1:L-1}}^\top
	\end{pmatrix} (4H)^{-1} \begin{pmatrix}
	\mathbf{0}_{U_{0:k-1}} \\ w_k \\\mathbf{0}_{U_{k+1:L-1}}
	\end{pmatrix} \leq \begin{pmatrix}
	\mathbf{0}_{U_{0:k-1}}^\top,w_k^\top, \mathbf{0}_{U_{k+1:L-1}}^\top
	\end{pmatrix} \widetilde{M}_k^{-1} \begin{pmatrix}
	\mathbf{0}_{U_{0:k-1}} \\ w_k \\\mathbf{0}_{U_{k+1:L-1}}
	\end{pmatrix} \\
	& = \begin{pmatrix}
	\mathbf{0}_{U_{0:k-1}}^\top,w_k^\top, \mathbf{0}_{U_{k+1:L-1}}^\top
	\end{pmatrix} \begin{pmatrix}
	M_{k-1}^{-1} - M_{k-1}^{-1} P_k S_k P_k^\top  M_{k-1}^{-1} & M_{k-1}^{-1} P_k S_k D_k^{-1} & 0 \\
	D_k^{-1} S_k P_k^\top M_{k-1}^{-1}  & D_k^{-1} - D_k^{-1} S_k D_k^{-1} & 0 \\
	0 & 0 & D_{t+1:L}^{-1}
	\end{pmatrix} \begin{pmatrix}
	\mathbf{0}_{U_{0:k-1}} \\ w_k \\\mathbf{0}_{U_{k+1:L-1}}
	\end{pmatrix} \\
	& = \begin{pmatrix}
	w_k^\top D_k^{-1} S_k P_k^\top ,w_k^\top N_k, \mathbf{0}_{U_{k+1:L-1}}^\top
	\end{pmatrix} \begin{pmatrix}
	\mathbf{0}_{U_{k-1}} \\ w_k \\\mathbf{0}_{U_{k+1:L-1}}
	\end{pmatrix} = w_k^\top N_k w_k 
	\end{split}
	\end{equation*}
	where the second line follows from Eq.~\eqref{eq:M_k_inv_decomp}.
\end{proof}

\begin{lemma} $N_k$ is positive definite.
\label{lem:N_pos}
\end{lemma}
\begin{proof} Since $(4H)^{-1}$ is positive definite, Lemma~\ref{lem:N_over_H} indicates that
	$ w_k^\top N_k w_k \geq 0 $ if $w_k$ is not zero vector, which finishes the proof.
\end{proof}

Notice that $\widetilde{P}_k = ( \mathbf{0}_{U_{0:k-1}\times U_k} ,P_k)$ where $\mathbf{0}_{U_{0:k-1}\times U_k}$ here refers to the zero matrix for $\fR^{U_{0:k-1}\times U_k}$. We have 
\begin{equation*}
\begin{pmatrix}
\mathbf{0}_{U_{0:k-1}\times U_k}^\top & P_k^\top 
\end{pmatrix} 
\begin{pmatrix}
M_{k-1}^{-1} - M_{k-1}^{-1} P_k S_k P_k^\top  M_{k-1}^{-1} & M_{k-1}^{-1} P_k S_k D_k^{-1}\\
D_k^{-1} S_k P_k^\top M_{k-1}^{-1}  & N_k
\end{pmatrix}   
\begin{pmatrix}
\mathbf{0}_{U_{0:k-1}\times U_k} \\ P_k
\end{pmatrix} = P_k^\top N_k P_k
\end{equation*}
which indicates a recursive formula of $N_k$ with respect to $D_k$,$P_k$,$C_k$ and $N_{k-1}$.

\begin{lemma} Due to the fact $N_k = ((C_k^{-1}+P_k^\top N_{k-1} P_k)^{-1} + D_k)^{-1}$, it holds that 
	$N_k \leq D_k^{-1}$ and $N_k \leq C_k^{-1}+P_k^\top N_{k-1} P_k$.
	\label{lem:inverse_matrix_formula}
\end{lemma}
\begin{proof}
	By Woodbury's Theorem, we have 
	$$S_k = D_k - D_k ( D_k + (C_k^{-1} +P_k^\top N_{k-1} P_k )^{-1})^{-1} D_k.$$
	Plugin it in the equation $N_k = D_k^{-1} - D_k^{-1} S_k D_k^{-1} $ yields the results.
\end{proof}

So far, we have generated a sequence of matrices $N_k\in \fR^{U_k \times U_k}$ that are positive-definite, greater than the projection of $(4H)^{-1}$ on $U_k$, and has a recursive formula which guarantees $N_k \leq C_k^{-1} +P_k^\top N_{k-1} P_k$. 

Let $R(s,a)\triangleq N_k\rbr{(s,a),(s,a)}$ denote the element at the row $(s,a)$ and column $(s,a)$ of matrix $N_k$ for all state-action pair $(s,a)\in U_k$. According to Lemma~\ref{lem:N_over_H}, we have $R(s,a)\geq (4H)^{-1}_{(s,a),(s,a)} = \frac{1}{4}H^{-1}_{(s,a),(s,a)}$. We then prove that the sum of $\frac{R(s,a)}{q(s,a)}$ can be bounded.

\begin{lemma} For the states in $S_k$ that $k>0$, $R(s,a)$ satisfies that
	\begin{equation}
\sum_{s \in S_k,a \in A}\frac{R(s,a)}{q(s,a)} \leq 2\rbr{\sqrt{L} + \frac{1}{\alpha L}} \sum_{s \in S_k}\sum_{a\neq \pi^\star(s)} q(s,a)^{1/2} + \rbr{ 1 + \frac{1}{L}} \sum_{s' \in S_{t-1},a'\in A}\frac{R(s',a')}{q(s',a')}.
	\end{equation}
	\label{lem:R_q_sum}
	Specifically, for the states in $S_0$, it holds that 
	$$ \sum_{s\in S_0,a\in A}\frac{R(s,a)}{q(s,a)} \leq 2\rbr{ \sqrt{L}+ \frac{1}{\alpha L}} \sum_{s\in S_0}\sum_{a\neq \pi^\star(s)}\sqrt{q(s,a)}. $$ 
\end{lemma}
\begin{proof} 
	For the $s = s_0 \in S_0$, we have 
	$R(s,a) \leq \min\cbr{q(s,a)^{3/2}, \frac{(q(s)-q(s,a))^{3/2} }{\alpha}}$. Thus, it holds that
	\begin{equation}
	\frac{R(s,a)}{q(s,a)}\leq \min\cbr{\sqrt{q(s,a)}, \frac{q(s)-q(s,a)}{\alpha \cdot q(s,a)}\sum_{a' \neq a}\sqrt{q(s,a)} }.
	\end{equation}
	Discussing the two cases $q(s,\pi^\star(s))\geq \frac{L}{L+1}q(s)$ and $q(s,\pi^\star(s))<\frac{L}{L+1}q(s)$ yields the proof of $t=0$.
	
	Then we consider states $s$ that $k(s) > 0 $. For notational convenience, let $R(s,a,s',a') = e_{s,a}^\top N_k e_{s',a'}$. Clearly, for $(s,a)\in U_k$ the $R(\cdot)$ forms the positive-definite matrix $N_k$. With the fact that $N_k\leq D_k^{-1}$, we have $R(s,a) \leq q(s,a)^{3/2}$. Moreover, by the fact $ w_k^\top N_k w_k \leq C_k^{-1} + P_k^\top N_{k-1} P_k $, we have 
	\begin{equation}
	\begin{split}
	R(s,a)  \leq & \frac{(q(s)-q(s,a))^{3/2} }{\alpha} + \sum_{s_1,a_1}\sum_{s_2,a_2}Pr(s|s_1,a_1)Pr(s|s_2,a_2)R(s_1,a_1,s_2,a_2) \\ 
	= & \frac{(q(s)-q(s,a))^{3/2} }{\alpha} \\ & + \sum_{s_1,a_1}\sum_{s_2,a_2}Pr(s|s_1,a_1)q(s_1,a_1)Pr(s|s_2,a_2)q(s_2,a_2)\frac{R(s_1,a_1,s_2,a_2)}{q(s_1,a_1)q(s_2,a_2)} \\ 
	\leq & \frac{(q(s)-q(s,a))^{3/2} }{\alpha} \\ & + \sum_{s_1,a_1}Pr(s|s_1,a_1)q(s_1,a_1)\rbr{\sum_{s_2,a_2}Pr(s|s_2,a_2)q(s_2,a_2)}\frac{R(s_1,a_1)}{q(s_1,a_1)^2} \\ 
	= & \frac{(q(s)-q(s,a))^{3/2} }{\alpha} + q(s)\sum_{s_1,a_1}Pr(s|s_1,a_1)\frac{R(s_1,a_1)}{q(s_1,a_1)}
	\end{split}
	\label{eq:apply_N_ineq}
	\end{equation}
	The third line follows from that the $T(s_1,a_1,s_2,a_2) = R(s_1,a_1,s_2,a_2)/q(s_1,a_1)q(s_2,a_2)$ forms a positive-definite matrix, and $|T(s_1,a_1,s_2,a_2)|\leq \frac{1}{2} (T(s_1,a_1) + T(s_2,a_2))$. In fact, we can construct the matrix $T$ by $T = Q N_k Q^\top$ where $Q = diag\cbr{q(s,a)^{-1}:(s,a)\in U_k}$. By Lemma~\ref{lem:N_pos} and the property of positive-definite matrices, we can infer that $T$ is positive-definite 
	as well.
	
	Then we discuss the bound for state $s$ in two cases. For the states that satisfies $q(s,\pi^\star(s)) \leq ( 1 - \frac{1}{L+1})q(s)$, in other words $q(s,\pi^\star(s)) \leq L \sum_{a\neq \pi^\star(s)} q(s)$,  all the sub-optimal actions $a \neq \pi^\star(s)$ satisfy that 
	\begin{equation}
	\label{eq:bound_non_optimal}
	\sum_{a \neq \pi^\star(s)}\frac{R(s,a)}{q(s,a)} \leq \sum_{a \neq \pi^\star(s)}\frac{q(s,a)^{3/2}}{q(s,a)} = \sum_{a \neq \pi^\star(s)}q(s,a)^{1/2}.
	\end{equation}
	And the optimal action $\pi^\star(s)$ satisfies that 
	\begin{equation}
	\label{eq:bound_optimal_case_1}
	\frac{R(s,\pi^\star(s))}{q(s,\pi^\star(s))} \leq q(s,\pi^\star(s))^{1/2} \leq \rbr{L \sum_{a \neq \pi^\star(s)}q(s,a)}^{1/2}\leq \sqrt{L}\sum_{a \neq \pi^\star(s)}q(s,a)^{1/2}.
	\end{equation}
	Combing Eq.~\eqref{eq:bound_non_optimal} and Eq.~\eqref{eq:bound_optimal_case_1} gives an upper bound of the term $\sum_{a}\frac{R(s,a)}{q(s,a)}$ as 
	\begin{equation}
	\label{eq:bound_rfunc_case_1}
	\sum_{a}\frac{R(s,a)}{q(s,a)} \leq \rbr{\sqrt{L}+1} \sum_{a \neq \pi^\star(s)}q(s,a)^{1/2}.
	\end{equation}
	On the other hand, for the states that satisfies $q(s,\pi^\star(s)) \geq ( 1 - \frac{1}{L+1})q(s)$, it holds that 
	\begin{equation}
	\label{eq:bound_optimal_case_2}
	\begin{split}
	\frac{R(s,a)}{q(s,a)} & \leq \frac{(q(s)-q(s,a))^{3/2}}{\alpha \cdot q(s,a)} + \frac{q(s)}{q(s,a)}\sum_{s_1,a_1}Pr(s|s_1,a_1)\frac{R(s_1,a_1)}{q(s_1,a_1)} \\
	& \leq \frac{q(s)-q(s,a)}{\alpha  \cdot q(s,a)}  \sum_{a \neq \pi^\star(s)}q(s,a)^{1/2} + \rbr{1 + \frac{1}{L}} \sum_{s_1,a_1}Pr(s|s_1,a_1)\frac{R(s_1,a_1)}{q(s_1,a_1)} \\ 
	& \leq \frac{1}{\alpha L}  \sum_{a \neq \pi^\star(s)}q(s,a)^{1/2} + \rbr{1 + \frac{1}{L}} \sum_{s_1,a_1}Pr(s|s_1,a_1)\frac{R(s_1,a_1)}{q(s_1,a_1)} 
	\end{split}
	\end{equation}
	where the second line follows from the fact $\rbr{q(s) - q(s,a)}^{1/2} \leq \sum_{a' \neq a} \sqrt{q(s,a')}$, and the third line uses the condition that $q(s,\pi^\star(s)) \geq L \rbr{q(s) - q(s,\pi^\star(s))}$. 
	
	By combing Eq.~\eqref{eq:bound_non_optimal} and Eq.~\eqref{eq:bound_optimal_case_2}, we show that 
	\begin{equation}
	\label{eq:bound_rfunc_case_2}
	\sum_{a}\frac{R(s,a)}{q(s,a)}  \leq \rbr{1+\frac{1}{\alpha L}} \sum_{a \neq \pi^\star(s)}q(s,a)^{1/2} + \rbr{1 + \frac{1}{L}} \sum_{s_1,a_1}Pr(s|s_1,a_1)\frac{R(s_1,a_1)}{q(s_1,a_1)}.
	\end{equation}
	Merge the upper bounds for these two cases in Eq.~\eqref{eq:bound_rfunc_case_1} and Eq.~\eqref{eq:bound_rfunc_case_2} shows that 
	\[
	\sum_{a}\frac{R(s,a)}{q(s,a)}  \leq 2\rbr{\sqrt{L} +\frac{1}{\alpha L} } \sum_{a \neq \pi^\star(s)}q(s,a)^{1/2} + \rbr{1 + \frac{1}{L}} \sum_{s_1,a_1}Pr(s|s_1,a_1)\frac{R(s_1,a_1)}{q(s_1,a_1)}.
	\]

	
	Therefore,by taking the summation of all state-action pairs in $U_k$, we have 
	\begin{equation}
	\begin{split}
	\sum_{s,a \in U_k} \frac{R(s,a)}{q(s,a)} & \leq 2\rbr{\sqrt{L} +\frac{1}{\alpha L} } \sum_{s \in S_k}\sum_{a\neq \pi^\star(s)} q(s,a)^{1/2} + \rbr{ 1 + \frac{1}{L}} \sum_{s \in S_k}\sum_{s' \in S_{k-1},a'\in A}Pr(s|s',a')\frac{R(s',a')}{q(s',a')} \\
	& =  2\rbr{\sqrt{L} +\frac{1}{\alpha L}} \sum_{s \in S_k}\sum_{a\neq \pi^\star(s)} q(s,a)^{1/2} + \rbr{ 1 + \frac{1}{L}} \sum_{s' \in S_{k-1},a'\in A}\frac{R(s',a')}{q(s',a')}
	\end{split}
	\end{equation}
\end{proof}

\begin{proof} (Lemma~\ref{lem:bound_term2_main})
	Denote the sum $\sum_{s,a \in U_k} \frac{R(s,a)}{q(s,a)}$ as $Q_k$. 
	By Lemma~\ref{lem:R_q_sum}, we have $$Q_k \leq 2\rbr{\sqrt{L} +\frac{1}{\alpha L} } \sum_{s \in S_k}\sum_{a\neq \pi^\star(s)}\sqrt{q(s,a)} + \rbr{1+\frac{1}{L}}Q_{k-1}.$$
	
	By using this relationship recursively, we have 
	\[
	\begin{split}
	Q_k \leq & 2\rbr{\sqrt{L} +\frac{1}{\alpha L} } \sum_{s \in S_k}\sum_{a\neq \pi^\star(s)}\sqrt{q(s,a)} + \rbr{1+\frac{1}{L}}Q_{k-1} \\ 
	\leq & 2\rbr{\sqrt{L} +\frac{1}{\alpha L} } \sum_{s \in S_k}\sum_{a\neq \pi^\star(s)}\sqrt{q(s,a)} \\
	& + 2\rbr{1+\frac{1}{L}}\rbr{\sqrt{L} +\frac{1}{\alpha L}} \sum_{s \in S_{k-1} }\sum_{a\neq \pi^\star(s)}\sqrt{q(s,a)} \\
	& +  \rbr{1+\frac{1}{L}}^2 Q_{k-2} \\ 
	\leq & 2\rbr{1+\frac{1}{L}}^{k}\rbr{\sqrt{L} +\frac{1}{\alpha L} } \sum_{l=0}^{k}\sum_{s \in S_l}\sum_{a\neq \pi^\star(s)}\sqrt{q(s,a)} \\
	\leq & 2e\rbr{\sqrt{L} +\frac{1}{\alpha L} } \sum_{l=0}^{k}\sum_{s \in S_l}\sum_{a\neq \pi^\star(s)}\sqrt{q(s,a)} 
	\end{split}
	\]
	where the last line applies the fact that $(1+\frac{1}{L})^{k} \leq (1+\frac{1}{L})^{L}\leq e$.
	Therefore, the Hessian matrix's inverse $H^{-1}$ satisfies that 
	$$\frac{1}{4}\sum_{s,a}\frac{H^{-1}_{(s,a)(s,a)}}{q(s,a)}\leq \sum_{k=0}^{L-1}Q_k\leq 2eL\rbr{\sqrt{L} +\frac{1}{\alpha L} } \sum_{s \in S}\sum_{a\neq \pi^\star(s)}\sqrt{q(s,a)}.$$
	Finally, we have 
	\begin{equation}
	\begin{split}
	\E\sbr{\norm{\hatl_t}_{\nabla^2\phi_{main}}^2} & = \E\sbr{\sum_{s,a}\sum_{s',a'}\frac{H^{-1}_{(s,a)(s',a')}}{q(s,a)q(s',a')}\Ind{s,a}\ell(s,a)\Ind{s',a'}\ell(s',a')}\\
	& \leq \E\sbr{\sum_{s,a}\rbr{\sum_{s',a'}\Ind{s',a'}\ell(s',a')}\frac{H^{-1}_{(s,a)(s,a)}}{q(s,a)^2}\Ind{s,a}\ell(s,a)} \\ 
	& \leq \E\sbr{\sum_{s,a}L\frac{H^{-1}_{(s,a)(s,a)}}{q(s,a)^2}\one_{s,a}\ell(s,a)} \\
	& \leq L \sum_{s,a}\frac{H^{-1}_{(s,a)(s,a)}}{q(s,a)} \leq 8eL^2 \rbr{\sqrt{L} +\frac{1}{\alpha L} }\sum_{s \in S}\sum_{a\neq \pi^\star(s)}\sqrt{q(s,a)}
	\end{split}
	\end{equation}
	where the second line follows from the similar idea in Eq.~\eqref{eq:apply_N_ineq} that constructs a positive definite matrix $T_{(s,a)(s',a')}=H^{-1}_{(s,a)(s',a')}/q(s,a)q(s',a')$, 
	the third line follows from the fact that the sum $\sum_{s',a'}\Ind{s',a'}\ell(s',a')\leq L$ since there are only $L$ steps in one episode where $\Ind{s',a'} = \Ind{s_{k(s')} = s',a_{k(s')} = a'}$.  
\end{proof}
Combing the above Lemma with the learning rates $\eta_t = \gamma \cdot \frac{1}{\sqrt{t}}$ finishes the proof of Lemma~\ref{lem:bound_term2}. 

\subsection{Proof of Theorem~\ref{thm:main}}

Although Lemma~\ref{lem:bound_term1} gives a bound of $\phi_{main}(q^\star) - \phi_{main}(q_t)$, the term  $\phi_{supp}(q^\star)-\phi_{supp}(q_1)$ could be infinity. Therefore, we want to find a valid occupancy measure $u$ with finite $\phi_{supp}(u)$ and close to $q^\star$.

The idea is analogous to the \textit{upper occupancy bound} in \citet{jin2019learning}. For each state-action pair $(s,a)$, there exist a policy that maximize the probability of visiting this pair under given transition function $P$. We denote $z(s,a)$ as the maximum probability of visiting state-action pair $(s,a)$, and $r^{s,a}\in \Omega$ as the corresponding occupancy measure. By Lemma~\ref{lem:convex_combine}, we know that $q_{exp} = \frac{1}{|S||A|}\sum_{s,a}r^{s,a}$ is a valid occupancy measure.  

We set $u = \rbr{1 - \frac{1}{T}}q^\star +  \frac{1}{T}\sum_{s,a}q_{exp}$ as the referrer occupancy measure, and prove that $u$ enjoys the following guarantees.

\begin{lemma} For $C=64L$, it holds that $\phi_{supp}(u)-\phi_{supp}(q_1) \leq 64L|S||A|\log(T|S||A|)$.
\label{lem:surogate_u_supp_bound}
\end{lemma} 
\begin{proof} According to the definition, we have 
\[
u = \rbr{1 - \frac{1}{T}}q^\star +  \frac{1}{T}\sum_{s,a}q_{exp} =  \rbr{1 - \frac{1}{T}}q^\star +  \frac{1}{T|S||A|}\sum_{s,a}r^{s,a}.
\]
Therefore, we have $u(s,a) \geq \frac{1}{T|S||A|}z(s,a)$ since $r^{s,a}(s,a) = z(s,a)$. By this fact, the $\phi_{supp}(u)-\phi_{supp}(q_1)$ can be bounded as 
\[
64L \sum_{s,a}\log\rbr{\frac{q_1(s,a)}{u(s,a)} } \leq 64L \sum_{s,a}\log\rbr{\frac{z(s,a)}{u(s,a)} } \leq 64L|S||A|\log(T|S||A|).
\]
\end{proof}

\begin{lemma} $\phi_{main}(u) - \phi_{main}(q^\star) \leq \frac{\rbr{1+\alpha} |S||A|}{T} $. 
\label{lem:surogate_u_main_bound}
\end{lemma}
\begin{proof}
\[
\begin{split}
& \phi_{main}(u) - \phi_{main}(q^\star) \\
= & \sum_{s,a} \rbr{ \sqrt{q^\star(s,a)}  + \alpha \sqrt{q^\star(s)-q^\star(s,a)} - \sqrt{u(s,a)} - \alpha \sqrt{u^\star(s)-u^\star(s,a)} } \\
=  & \sum_{s,a} \rbr{  \sqrt{q^\star(s,a)}   - \sqrt{\frac{T-1}{T}q^\star(s,a) + \frac{q_{exp}(s,a) }{T} } } \\
& +  \sum_{s,a} \alpha  \rbr{  \sqrt{q^\star(s)-q^\star(s,a)}- \sqrt{\frac{T-1}{T}(q^\star(s)-q^\star(s,a)) + \frac{q_{exp}(s)-q_{exp}(s,a) }{T} } } \\
\leq & \rbr{1 - \sqrt{\frac{T-1}{T}} }\sum_{s,a} \rbr{ \sqrt{q^\star(s,a)}  +  \alpha  \sqrt{q^\star(s)-q^\star(s,a)} } \\ 
\leq & \frac{\rbr{1+\alpha} |S||A|}{T} 
\end{split}
\]
where the third line follows from the fact that $q_{exp}(s) \geq 0$. 
\end{proof}

\begin{lemma} $\Reg(q^\star) - \Reg(u) = \E\sbr{\sum_{t=1}^{T}\inner{u-q^\star, \hatl_t}} \leq L$. 
	\label{lem:surogate_u_reg_bound}
\end{lemma}
\begin{proof}
\[
\begin{split}
\E\sbr{\sum_{t=1}^{T}\inner{u-q^\star, \hatl_t}} & = \frac{1}{T} \E\sbr{\sum_{t=1}^{T}\inner{q_{exp}-q^\star, \hatl_t}} \\
& = \frac{1}{T}\inner{q_{exp}-q^\star,\sum_{t=1}^{T}\ell_t} \\
& \leq \frac{1}{T} \norm{q_{exp}-q^\star}_1 \norm{\sum_{t=1}^{T}\ell_t}_{\infty} \leq \frac{LT}{T} = L 
\end{split}
\]
\end{proof}

\begin{proof}(Theorem~\ref{thm:main}) By Lemma~\ref{lem:ftrl_main},~\ref{lem:surogate_u_supp_bound},~\ref{lem:surogate_u_reg_bound} and \ref{lem:surogate_u_main_bound}, we have 
\begin{equation}
\begin{split}
\Reg_T(q^\star) = & \Reg_T(u) + \Reg(q^\star) - \Reg(u) \\ 
 \leq & \sum_{t=1}^{T}(\eta_t^{-1} - \eta_{t-1}^{-1})\rbr{\phi_{main}(q^\star) - \phi_{main}(q_t)} + 8\sum_{t=1}^{T}\E\sbr{\norm{\hatl_t}_{\nabla^{-2}\psi_t(q_t)}} \\
& +\phi_{supp}(u) - \phi_{supp}(q_1) + \sum_{t=1}^{T}(\eta_t^{-1} - \eta_{t-1}^{-1})\rbr{\phi_{main}(u) - \phi_{main}(q^\star)} + L\\ 
\leq & \sum_{t=1}^{T}(\eta_t^{-1} - \eta_{t-1}^{-1})\rbr{\phi_{main}(q^\star) - \phi_{main}(q_t)} + 8\sum_{t=1}^{T}\E\sbr{\norm{\hatl_t}_{\nabla^{-2}\psi_t(q_t)}} \\
& + 64L|S||A|\log(T|S||A|) + \frac{\rbr{1+\alpha}|S||A|}{\gamma \sqrt{T}} + L.
\end{split}
\label{eq:main_with_term1and2}
\end{equation}
By the asymptotic inequality of $T$ that $T^{-1/2} = o\rbr{\log T}$, the terms in the second line can be bounded as $O(L|S||A|\log(T|S||A|)$. 


Plugging Lemma~\ref{lem:bound_term1} and ~\ref{lem:bound_term2} finished the proof of Theorem~\ref{thm:main}
\[
\begin{split}
Reg_T \leq & \cbr{\frac{1+\alpha}{\gamma} + 64eL^2 \rbr{\sqrt{L} + \frac{1}{\alpha L}} \gamma } \sum_{t=1}^{T}\sum_{s\in S,a\neq \pi^\star(a)}\sqrt{\frac{q_t(s,a)}{t}} \\ 
& + \frac{\rbr{1 + \alpha|A|}\sqrt{|S|L}}{\gamma}  \sum_{t=1}^{T}\sqrt{\sum_{s\in S,a\neq \pi^\star(a)}\frac{q_t(s,a)}{t}} \\ 
& + \order\rbr{L|S||A|\log(T|S||A|)}.
\end{split}
\]
\end{proof}


\subsection{Proof of Theorem~\ref{thm:adversarial_another}}
Recall the Eq.~\eqref{eq:main_with_term1and2} in the proof of Theorem~\ref{thm:main}
\[
\begin{split}
\Reg_T(q^\star) \leq & \sum_{t=1}^{T}(\eta_t^{-1} - \eta_{t-1}^{-1})\rbr{\phi_{main}(q^\star) - \phi_{main}(q_t)} + 8\sum_{t=1}^{T}\E\sbr{\norm{\hatl_t}_{\nabla^{-2}\psi_t(q_t)}} \\
& + \order\rbr{L|S||A|\log(T|S||A|)}.
\end{split}
\]

We then introduce the bounds of the term $1$ and $2$ without self-bounding terms $\sum_{a\neq a^\star}\sqrt{q_t(s,a)}$. 

\begin{lemma}
	\label{lem:bound_term1_another} (Bound of Term $1$) By setting $\eta_t = \gamma \cdot \frac{1}{\sqrt{t}}$, It holds that 
	\begin{equation}
	\sum_{t=1}^{T}(\eta_t^{-1} - \eta_{t-1}^{-1})\rbr{\phi_{main}(q^\star) - \phi_{main}(q_t)} \leq \frac{4\rbr{1 + \alpha\sqrt{A}}}{\gamma}\sqrt{L|S||A|T}.
	\end{equation}
\end{lemma}

\begin{proof} 
	By Lemma~\ref{lem:phi_decompo_1}, we have 
\[
\begin{split}
& \phi_{main}(q^\star) - \phi_{main}(q_t) \\ 
\leq &  (1+\alpha) \sum_{s\in S\setminus\{s_L\}}\sum_{a \in A, a \neq \pi^{\star}(s)}\sqrt{q_t(s,a)}  + \rbr{ 1 + (|A|-1)\alpha}\sum_{s\in S}\rbr{\sqrt{q_t(s)} - \sqrt{q^\star(s)}}   \\ 
\leq &  (1+\alpha)\sqrt{L|A||S|} + \rbr{ 1 + (|A|-1)\alpha}\sqrt{|S|L} \\
\leq & 2\rbr{1 + \alpha\sqrt{A}} \sqrt{L|S||A|}.
\end{split}
\]
where the second line follows from the facts that $\sum_{s,a}q_t(s,a) = L$, $\sum_{s,a}q_t(s)=L$ and H\"older's inequality. Notice that $\eta_t^{-1} - \eta_{t-1}^{-1} \leq \frac{\sqrt{t}}{\gamma}$, combining the above inequality with the fact that $\sum_{t=1}^{T}\frac{1}{\sqrt{t}} \leq 2\sqrt{T}$ yields the proof.  
\end{proof}


\begin{lemma}
	\label{lem:bound_term2_another} (Bound of Term $2$) For $\hatl_t$ such that $0\leq \hatl_t = \frac{\ell_t(s,a)\Ind{s_{k(s)}=s,a_{k(s)}=a}}{q(s,a)} \leq \frac{1}{q(s,a)}$ where $q\in\Omega$, it holds that 
	\begin{equation}
	\sum_{t=1}^{T}\E\sbr{\norm{\hatl_t}^2_{\nabla^{-2} \psi_t(q_t)}} \leq 64\gamma\sqrt{L|S||A|T}.
	\end{equation} 
\end{lemma}

\begin{proof} 
	By the fact that $H^{-1} \leq diag\cbr{4q(s,a)^{3/2}:s\in S,a\in A}$, we have 
	\begin{equation}
	\begin{split}
	\E\sbr{\norm{\hatl_t}_{\nabla^2\phi_{main}}^2} & = \E\sbr{\sum_{s,a}\sum_{s',a'}\frac{H^{-1}_{(s,a)(s',a')}}{q(s,a)q(s',a')}\Ind{s,a}\ell(s,a)\Ind{s',a'}\ell(s',a')}\\
	& \leq \E\sbr{\sum_{s,a} \frac{4q(s,a)^{3/2}}{q(s,a)^2}\Ind{s,a}\ell(s,a)} \\ 
	& = 4\sum_{s,a} \sqrt{q(s,a)} \ell(s,a) \\
	& \leq 4 \sum_{s,a} \sqrt{q(s,a)} \\ 
	& \leq 4 \sqrt{L|S||A|}
	\end{split}
	\label{eq:phi_main_another}
	\end{equation}
	where the second line follows from the fact that $H^{-1} \leq diag\cbr{4q(s,a)^{3/2}:s\in S,a\in A}$,  the third line and forth line utilize the properties that $\E\cbr{\Ind{s,a}}=q(s,a)$ and $\ell(s,a)\in [0,1]$, the last line is derived by that $\sum_{s,a} q(s,a)=L$ and H\"older's inequality. 
	
	Combing Eq.~\eqref{eq:phi_main_another} with the fact that $\sum_{t=1}^{T}\frac{1}{\sqrt{t}} \leq  2\sqrt{T} $ finishes the proof. 
\end{proof}

Plugging Lemma~\ref{lem:bound_term1_another} and Lemma~\ref{lem:bound_term2_another} finishes the proof of Theorem~\ref{thm:adversarial_another} that 
\[
\Reg_T(q^\star) \leq \rbr{\frac{4\rbr{1 + \alpha\sqrt{A}}}{\gamma} + 64\gamma} \sqrt{L|S||A|T} + \order\rbr{L|S||A|\log(T|S||A|)}. 
\]



==> main_result.tex <==
%!TEX root=main.tex
\section{Main Results}
\label{sec:result}

To present the regret guarantees achieved by our algorithm, we introduce the certain \textit{self-bounding} property that leads to the best of both worlds result.  

\begin{theorem}
\label{thm:main}
(Self-bounding Property)For $C=64L$ and $\eta_t= \gamma \cdot \frac{1}{\sqrt{t}}$, our algorithm ensures
\begin{equation}
\label{eq:main}
	\begin{split}
Reg_T \leq & \cbr{\frac{1+\alpha}{\gamma} + 64eL^2 \rbr{\sqrt{L} + \frac{1}{\alpha L}} \gamma } \sum_{t=1}^{T}\sum_{s\in S,a\neq \pi^\star(a)}\sqrt{\frac{q_t(s,a)}{t}} \\ 
& + \frac{\rbr{1 + \alpha|A|}\sqrt{|S|L}}{\gamma}  \sum_{t=1}^{T}\sqrt{\sum_{s\in S,a\neq \pi^\star(a)}\frac{q_t(s,a)}{t}} \\ 
& + \order\rbr{L|S||A|\log(T|S||A|)}.
\end{split}
\end{equation}
\end{theorem}

Based on this property, we have the following result 
\begin{corollary} \label{col:eval} By setting $C=64L$, $\eta_t =\gamma \cdot \frac{1}{\sqrt{t}}$, our algorithm ensures that in the stochastic cases 
	\begin{equation}
	\label{eq:main_eval}
	\begin{split}
	Reg_T \leq &  4\cbr{\frac{1+\alpha}{\gamma} + 64eL^2 \rbr{\sqrt{L} + \frac{1}{\alpha L}} \gamma }^2 \sum_{s\in S\setminus \{s_L\}, a \neq \pi^\star{s} }\frac{\log T}{ \gap(s,a) }  \\ 
	& + 4 \cbr{\frac{\rbr{1 + \alpha|A|}\sqrt{|S|L}}{\gamma} }^2 \frac{\log T}{\gap_{min}} \\ 
	& + \order\rbr{L|S||A|\log(T|S||A|)}.
	\end{split}
	\end{equation}
where $\gap_{min} = \min_{s\in S\setminus \{s_L\}, a \neq \pi^\star{s} } \gap(s,a)$.
\end{corollary}
 
\begin{proof}
For notation convenience, we set two constants $U=\cbr{\frac{1+\alpha}{\gamma} + 64eL^2 \rbr{\sqrt{L} + \frac{1}{\alpha L}} \gamma }$ and $V=\frac{\rbr{1 + \alpha|A|}\sqrt{|S|L}}{\gamma} $. In the stochastic case, with the fact that $x\sqrt{\frac{q_t(s,a)}{t}}\leq \frac{1}{2}\rbr{ \frac{\gap(s,a)q_t(s,a)}{2} + \frac{4x^2}{t\gap(s,a)}}$ holds for any $x>0$, we have 
\[
\begin{split}
U\sum_{t=1}^{T}\sum_{s\in S,a\neq \pi^\star(a)}\sqrt{\frac{q_t(s,a)}{t}} & \leq \sum_{t=1}^{T}\sum_{s\in S,a\neq \pi^\star(a)}\frac{4U^2}{2t\gap(s,a)} +  \sum_{t=1}^{T}\sum_{s\in S,a\neq \pi^\star(a)}\frac{\gap(s,a)q_t(s,a)}{4} \\
& \leq \frac{4U^2}{2} \sum_{s\in S,a\neq \pi^\star(a)}\frac{\log T}{\gap(s,a)} + \frac{1}{4}Reg_T
\end{split}
\] 
where the last line uses Eq~\ref{eq:regdef_gap}.

Similarly, we have 
\[
\begin{split}
V \sum_{t=1}^{T}\sqrt{\sum_{s\in S,a\neq \pi^\star(a)}\frac{q_t(s,a)}{t}} & \leq \sum_{t=1}^{T}\frac{4V^2}{2t\gap_{min}(s,a)} +  \sum_{t=1}^{T}\sum_{s\in S,a\neq \pi^\star(a)}\frac{\gap_{min}q_t(s,a)}{4} \\
& \leq \frac{4V^2}{2} \cdot \frac{\log T}{\gap(s,a)} + \frac{1}{4}Reg_T.
\end{split}
\] 

Plugging these inequalities in Eq~\ref{eq:main_eval} yields
\[
\begin{split}
\rbr{1 - \frac{1}{4} - \frac{1}{4}}Reg_T & \leq \frac{4U^2}{2} \sum_{s\in S,a\neq \pi^\star(a)}\frac{\log T}{\gap(s,a)}  + \frac{4V^2}{2} \cdot \frac{\log T}{\gap(s,a)} + \order\rbr{L|S||A|\log(T|S||A|)} \\
\xRightarrow{}    Reg_T &\leq 4U^2 \sum_{s\in S,a\neq \pi^\star(a)}\frac{\log T}{\gap(s,a)} + \frac{4V^2\log T}{\gap(s,a)} + \order\rbr{L|S||A|\log(T|S||A|)}.
\end{split}
\]
To decide the value of parameters $\alpha$ and $\gamma$, we consider the worst cases that all $\gap(s,a) = \gap_{min}$ for all sub-optimal state-action pairs, and minimize the order of $\gap_{min}$ in the bound. In other words, the parameters should minimize the value of $4|S||A|U^2 + 4V^2$, which can be decomposed as 
\[
\begin{split}
& 4|S||A|U^2 + 4V^2 \\
= & 4|S||A|\cbr{\frac{1+\alpha}{\gamma} + 64eL^2 \rbr{\sqrt{L} + \frac{1}{\alpha L}} \gamma }^2  + 4|S| \cbr{\frac{\rbr{1 + \alpha|A|}\sqrt{L}}{\gamma}}^2 \\
\leq & 8|S| \cdot \frac{\rbr{1+\alpha}^2 |A| + \rbr{1 + \alpha|A|}^2 L }{\gamma^2} + 8|S||A| \cdot \rbr{64e}^2 L^4 \rbr{\sqrt{L} + \frac{1}{\alpha L}}^2 \gamma^2 \\
\leq & 16|S| \cdot \frac{|A| + L + 2\alpha^2|A|^2 L }{\gamma^2} + 16|S||A| \cdot \rbr{64e}^2 L^4 \rbr{L + \frac{1}{\alpha^2 L^2}} \gamma^2
\end{split}
\]
where the second line and the third line follow from the inequality that $x^2 + y^2 \leq (x+y)^2\leq 2(x^2+y^2)$ for $x,y\geq0$ and the fact that $ L \geq 1$.

Clearly, the optimal choice of $\gamma$ would satisfy $$\gamma = \sqrt[4]{\frac{16|S|\rbr{|A| + L + 2\alpha^2|A|^2 L}}{16|S||A|\rbr{64e}^2 L^4 \rbr{L + \frac{1}{\alpha^2 L^2}}} }.$$ Therefore, our goal is to simplify the following term as 
\[
\begin{split}
& \sqrt{256|S|^2|A|\rbr{|A| + L + 2\alpha^2|A|^2 L}\rbr{64e}^2 L^4 \rbr{L + \frac{1}{\alpha^2 L^2}} }\\
= & 1024e|S|L^2\sqrt{|A|L\rbr{|A| + L }} \sqrt{\rbr{1 + \alpha^2\frac{2|A|^2 L}{|A|+L}}\rbr{1 + \frac{1}{\alpha^2 L^3}}} \\
\end{split}
\]
For the minimization problem of the format $\rbr{1 + a x }\rbr{1  + \frac{b}{x}}$, we can verify that $x = \sqrt{\frac{b}{a}}$ is the optimal point.
Therefore, by setting $\alpha = \sqrt[4]{\frac{|A|+L}{L^3 \cdot 2|A|^2L}} = \sqrt[4]{\frac{|A|+L}{2|A|^2L^4} } $ , we have 
$$ \gamma =  \sqrt[4]{\frac{16|S|\rbr{|A|+L}\rbr{1+ \alpha^2 \cdot \frac{2|A|^2 L}{|A|+L}}}{16|S||A|\rbr{64e}^2 L^5 \rbr{1 + \frac{1}{\alpha^2 L^3}}} }=   \sqrt[4]{\frac{\rbr{|A|+L}}{|A|\rbr{64e}^2 L^5} }.$$

Plugging these parameters in $U$ and $V$, we have 
\[
\begin{split}
4U^2 = & 4 \cbr{\frac{1+\alpha}{\gamma} + 64eL^2 \rbr{\sqrt{L} + \frac{1}{\alpha L}} \gamma }^2 \\
\leq &  \frac{16}{\gamma^2} + 16\rbr{64e}^2L^4 \rbr{ L + \frac{1}{L^2} \cdot \sqrt{\frac{2|A|^2L^4}{|A|+L}} } \gamma^2 \\ 
= & 1024 \sqrt{\frac{|A|L^5}{|A|+L}} + 1024L^4\sqrt{\frac{|A|+L}{|A|L^5}} \rbr{ L +  \frac{1}{L^2} \cdot \sqrt{\frac{2|A|^2L^4}{|A|+L}} } \\
= & 1024L^2 \sqrt{\frac{|A|L}{|A|+L}} + 1024L^2\sqrt{\frac{|A|+L}{|A|L}} \rbr{ L +   \sqrt{\frac{2|A|^2}{|A|+L}} } \\
= & 1048L^2 \rbr{  \sqrt{\frac{|A|L}{|A|+L}}  + \sqrt{\frac{L|A|+L^2}{|A|}} +   \sqrt{\frac{2|A|}{L}} } \\
\leq & 1048L^2 \rbr{ \min\cbr{\sqrt{A},\sqrt{L}} + \sqrt{L} + \frac{L}{\sqrt{A}} + 2\sqrt{A} } \\
= & \order\rbr{L^2\rbr{\sqrt{A}+\sqrt{L}+\frac{L}{\sqrt{A}}}}  ,
\end{split}
\]
and 
\[
\begin{split}
4V^2 = & 4|S| \cbr{\frac{\rbr{1 + \alpha|A|}\sqrt{L}}{\gamma}}^2  = 4|S|L \frac{ \rbr{1  + \alpha |A|}^2 }{ \gamma^2} \\
\leq &  8\cdot 64e|S|L \rbr{1  +  |A|^2 \sqrt{\frac{|A|+L}{2|A|^2L^4}} } \sqrt{\frac{|A|L^5}{|A|+L}}\\ 
= & 512e|S|L \rbr{ L^2\sqrt{\frac{|A|L}{|A|+L}} + |A| \sqrt{\frac{|A|+L}{2L^4}} \sqrt{\frac{|A|L^5}{|A|+L}} } \\
\leq & 512e|S|L \rbr{ L^2\sqrt{A} + |A|^{3/2}\sqrt{L} } \\
= & \order\rbr{|S|L \rbr{ L^2\sqrt{A}+ |A|^{3/2}\sqrt{L} }}.
\end{split}
\]
\end{proof}

Clearly, by the concavity of $\sqrt{x}$ and the fact  $\sum_{s\in S,a\neq \pi^\star(a)} q_t(s,a) \leq L$, we have $\sum_{s\in S,a\neq \pi^\star(a)} \sqrt{q_t(s,a)}\leq \sqrt{L|S||A|}$. Plugging it in Eq~\ref{eq:main} can yield a regret bound in adversarial cases. However, comparing with the yielded bound, our algorithm can achieve a better result.
\begin{theorem} 
	\label{thm:adversarial_another}
	For $C=64L$, $\eta_t= \gamma \cdot \frac{1}{\sqrt{t}}$, we have 
	\begin{equation}
	\label{eq:adversarial_another}
	Reg_T \leq \rbr{\frac{4\rbr{1 + \alpha\sqrt{|A|}}}{\gamma} + 64\gamma} \sqrt{L|S||A|T} + \order\rbr{L|S||A|\log(T|S||A|)}.
	\end{equation}
\end{theorem}

By Theorem~\ref{thm:adversarial_another}, our algorithm with the setting described in Corollary~\ref{col:eval} ensures a bound on the coefficient of $\sqrt{L|S||A|T}$ as  
\[
\begin{split}
 &\rbr{\frac{4\rbr{1 + \alpha\sqrt{|A|}}}{\gamma} + 64\gamma}\\
= & \rbr{1 + \sqrt[4]{\frac{|A|+L}{2L^4} } }\sqrt[4]{\frac{|A|\rbr{64e}^2 L^5}{\rbr{|A|+L}} } + 64  \sqrt[4]{\frac{\rbr{|A|+L}}{|A|\rbr{64e}^2 L^5} } \\
\leq & 16 \sqrt[4]{\frac{|A|L^5}{\rbr{|A|+L}} } + 16 \sqrt[4]{\frac{|A| L^5}{\rbr{2L^4}} } + 8 \sqrt[4]{\frac{\rbr{|A|+L}}{|A|L^5} } \\
\leq & 16 |A|^{1/4}L + 16 |A|^{1/4}L^{1/4} + 16 \\  
= & \order\rbr{ |A|^{1/4}L }.
\end{split}
\]

==> problem_setting.tex <==
%!TEX root=main.tex
\section{Problem Setup and Notations}
\label{sec:probform}
% Makrov Decision Process 
A Markov decision process is defined by a tuple $(S,A,P, \{\ell_t\}_{t=1}^T)$, 
where $S$ is the finite state space, $A$ is the finite action space, $P:S \times A \times S \rightarrow [0,1]$ is the transition function, with $P(s'|s,a)$ being the probability of transferring to state $x'$ when executing action $a$ in state $s$,
and $\ell_t: S\times A\rightarrow [0,1]$ is the loss function for episode $t$. 

% Episodic Loop-free Architecture 
Throughout this paper, we consider an episodic setting with a given finite horizon $L$, and assume the states has a layered structure satisfying the following conditions:
\begin{itemize}
	\item The state space $S$ consists of $L+1$ layers $S_0, \ldots, S_L$ such that $S$ = $\bigcup_{k=0}^{L}S_k$ and $S_i \cap S_j = \emptyset$ for $i\neq j$.
	\item $S_0$ and $S_L$ are singletons, that is, $S_0 = \{s_0\}$ and $S_L = \{s_L\}$.
	\item Transitions are possible only between consecutive layers. In other words, if $P(s'|s,a) > 0$, then $s' \in S_{k+1}$ and $x\in S_k$ for some $k$. 
\end{itemize}

% interaction protocal 
Ahead of time, the environment decides a MDP and the state space $S$ with its layer-structure, the action space $A$ and the transition function are known to the learner.  The interaction proceeds in $T$ episodes. Simultaneously with the loss is generated either by the random variables or by an adversary, the learner starts at stater $s_0$ and decides a stochastic policy $\pi_t: S \times A \rightarrow  [0,1]$, where $\pi_t(a|s)$ is the probability of taking action $a$ at the given state $s$, therefore $\sum_{a}\pi_t(s,a)=1$ for all state $s$. Then the learner executes the policy until reaching the final state $s_L$, visiting $L$ state-action pairs $(s_0, a_0), \ldots, (s_{L-1}, a_{L-1})$, where the learner draws action $a_k$ from $\pi_t(\cdot| s_k)$ and the environment draw the next state $s_{k+1}$  from $P(\cdot|s_k,a_k)$ for step $k = 0,\ldots,L-1$. 

% Loss definition 
For any given policy $\pi$, we denote its expected loss in episode $t$ as 
\[
\mathbb{E}\left[\left.\sum_{k=0}^{L-1}\ell_t(s_k,a_k)\right| P,\pi\right],
\]
where the notation $\mathbb{E}[\cdot|P,\pi]$ emphasizes that the state-action pairs $(s_0, a_0), \ldots, (s_{L-1}, a_{L-1})$ are random variables generated according to the transition function $P$ and a stochastic policy $\pi$. The total loss is 
The total loss over $T$ episodes for any fixed policy $\pi$ is thus
\[
L_T(\pi) = \sum_{t=1}^{T}\mathbb{E}\left[\left.\sum_{k=0}^{L-1}\ell_t(s_k,a_k)\right| P,\pi\right],
\]
while the total loss of the learner is
\begin{equation*}
\begin{split}
L_T & = \sum_{t=1}^{T}\mathbb{E}\left[\left.\sum_{k=0}^{L-1}\ell_t(s_k,a_k)\right| P,\pi_t\right].
\end{split}
\end{equation*}
The regret with respect to a policy is defined as $R_T(\pi) = L_T - L_T(\pi)$. The goal of the learner is to minimize the regret with respect to the optimal policy, defined as
\[
Reg_T = L_T - \min_{\pi}L_T(\pi)
\]
where $\pi$ ranges over all stochastic policies. We denote $\pi^\star =  \argmin_{\pi}L_T(\pi)$ as the optimal policy in hindsight. Clearly, the optimal policy $\pi^\star$ is deterministic. Therefore, we abuse the notation $\pi^\star$ to define the optimal action at state $s$ as $\pi^\star(s)$. 

\paragraph{Assumption on Reachability.} In this paper, we assume every state is reachable. That is, for every state $s$, there exists a policy $\pi$ such that the probability of reaching $s$ under $\pi$, $Pr(s_{k(s)} = s | P,\pi)$,  is non-zero. However, this assumption can be dropped by removing the unreachable states with the help of given transition function $P$ before the interaction starts. 

\paragraph{General Notation.} \label{para:general_notation}
We use $k(s)$ to denote the index of the layer to which state $s$ belongs, and $\Ind\{\cdot\}$ to denote the indicator function whose value is $1$ if the input holds true and $0$ otherwise.
Let $o_t = \{(s_k, a_k, \ell_t(s_k, a_k))\}_{k=0}^{L-1}$ be the observation of the learner in episode $t$,
and $\calF_t$ be the $\sigma$-algebra generated by $(o_1, \ldots, o_{t-1})$.
Also let $\E_t[\cdot]$ be a shorthand of $\E[\cdot | \calF_{t}]$. For a positive definite matrix $M \in \fR^{ K \times K}$, we denote norm $\norm{x}_M \triangleq \sqrt{ x^\top M x}$ for any vector $x\in \fR^{K}$.  For two matrices $M_1$ and $M_2$, $M_1 \leq M_2$ means that $M_2 - M_1$ is positive semi-definite. We use $|S|$, $|A|$ denote the size of state set $S$ and action set $A$.  We denote $S_{0:k}\triangleq\bigcup_{\tau=0}^{k}S_\tau$ as the states in layer $0$ to layer $k$,  $U_k=S_k\times A$ as the set of the state-action pairs of layer $t$, and  $U_{0:k}=S_{0:k}\times A$ as the state-action pairs from layer $0$ to layer $k$.


\paragraph{Matrix Notation.} \label{para:matrix_notation} By convention,  we arrange all state-action pairs in an ascending order of layer index, and break ties by first state index and then action index. This order forms a one-one mapping from $S\times A$ to $[|S||A|] = \cbr{1,\ldots,|S||A|}$, which allows us to place the second-order derivatives into the matrix in $\fR^{|S||A| \times |S||A|}$. By the aforementioned order of state-action pairs, we denote $\fR^{D \times E}$ for a set $D,E\subset S\times A$ as the set of matrices in the shape of $|D|\times |E|$. 

We denote $M_{(s,a),(x,b)}$ and $M\rbr{(s,a),(x,b)}$ as the element at the row associated with $(s,a)$ and the column associated with $(x,b)$,  for all matrices $M\in \fR^{D \times E}$ and all state-action pairs $(s,a)\in D$, $(x,b)\in E$. In addition, we force such alignment while extending a matrix $M\in \fR^{D \times E}$ to a new matrix $M'\in \fR^{D' \times E'}$ where $D \subset D', E\subset E'$ by adding zeros. In other words, it holds that $M_{(s,a),(x,b)} = M'_{(s,a),(x,b)}$ for all $(s,a)\in D$ and $(x,b)\in E$. Similarly, we define the $\fR^{D}$ and denote the element at the row for $(s,a)$ by $w(s,a)$ for any vector in $w\in\fR^{D}$.



\subsection{Occupancy Measures}
\label{sec:occupancy}

Solving the problem with techniques from online learning requires introducing the concept of \textit{occupancy measures}.
Specifically, the occupancy measure $q^{P,\pi}: S \times A \rightarrow [0,1]$ associated with a stochastic policy $\pi$ and a transition function $P$ is defined as follows:
\[
q^{P,\pi}(s,a) = \Pr\left[s_k=s,a_k=a \;|\; P,\pi\right] 
\]
where $k=k(s)$ is the index of the layer to which $x$ belongs.
In other words, $q^{P,\pi}(s,a)$ is the marginal probability of encountering the state-action pair $(s, a)$ when executing policy $\pi$ in a MDP with transition function $P$. 

Clearly, an occupancy measure $q$ satisfies the following two properties.
First, due to the loop-free structure, each layer is visited exactly once and thus for every $k = 0, \ldots, L-1$,
\begin{equation}
\sum_{s\in S_k}\sum_{a\in A}q(s,a) = 1. 
\label{eq:1}
\end{equation}
Second, the probability of entering a state when coming from the previous layer is exactly the probability of leaving from that state to the next layer (except for $s_0$ and $s_L$). Therefore, for every $k = 1, \ldots, L-1$ and every state $s\in S_k$, we have 
\begin{equation}
\sum_{s'\in S_{k-1}}\sum_{a'\in A}q(s',a)Pr(s|s',a') = \sum_{a}q(s,a).
\label{eq:2}
\end{equation}

It turns out that these two properties are also sufficient for any function $q: S\times A \rightarrow [0,1]$ to be an occupancy measure associated with the given transition $P$ function and some policy. 

\begin{lemma}[\citet{zimin2013}]
	\label{lem:occupancy_measure}
	If a function $q: S\times A \rightarrow[0,1]$ satisfies conditions~\eqref{eq:1} and~\eqref{eq:2}, then it is a valid occupancy measure associated with given transition function $P$ and the following induced policy $\pi^q$:
	\begin{equation*}
	\begin{split}
	\pi^q(a|s) & = \begin{cases} \frac{q(s,a)}{\sum_{b\in A}q(s,b)} , &\sum_{b\in A}q(s,b)>0 \\ 0, &\sum_{b\in A}q(s,b) = 0  \end{cases}
	\end{split}
	\end{equation*}
\end{lemma}

Through out this paper, we denote  $\Omega$ as the set of all valid occupancy measure of given transition function $P$. With the concept of occupancy measure, we can reduce the problem of learning a policy to the problem of learning an occupancy measure and apply online linear optimization techniques. The expected loss of following a policy $\pi$ for episode $t$ can be rewritten as
\begin{equation*}
\begin{split}
&\mathbb{E}\left[\left.\sum_{k=0}^{L-1}\ell_t(s_k,a_k)\right|P,\pi\right] \\
= & \sum_{k=0}^{L-1}\sum_{s\in S_k}\sum_{a\in A} q^{P,\pi}(s,a) \ell_t(s,a) \\
=  &\sum_{s\in S\setminus \{s_L\}, a\in A}q^{P,\pi}(s,a)\ell_t(s,a) \triangleq  \langle q^{P,\pi}, \ell_t\rangle,
\end{split}
\end{equation*}
% 
and accordingly the regret of the learner can also be rewritten as
\begin{equation}
\label{eq:regdef}
Reg_T = L_T - \min_{\pi}L_T(\pi) = \sum_{t=1}^T \langle q^{P,\pi_t} - q^\star, \ell_t \rangle
\end{equation}
where $q^\star \in \argmin_{q\in\Omega} \sum_{t=1}^T\langle q,\ell_t\rangle$ is the optimal occupancy measure in $\Omega$. Accordingly, it's also the occupancy measure associated with the optimal policy $\pi^\star$. 

\subsection{Sub-Optimality Gaps}
\label{sec:gap}
% Best-of-both-worlds 
The loss function can be either generated \textit{stochastically} or \textit{adversarially}. In the \textit{stochastic} case, we assume that $\ell_1,\ldots,\ell_T$ are i.i.d samples from a fixed unknown distribution over $[0,1]$. We use $\bar{\ell}:S \times A \rightarrow [0,1]$ to denote the expected loss function. To achieve a more favorable regret form $C\log T$ where $C$ is a problem-dependent constant, we introduce the \textit{sub-optimality gaps} which are defined as 
\begin{equation}
\label{eq:gapdef}
\gap(s,a) = V^{\pi^\star}(s) - Q^{\pi^\star}(s,a),
\end{equation}
where $\pi^\star$ denote the optimal policy and $V^{\pi^\star}$ and $Q^{\pi^\star}$ denote the value and Q functions with respect to $\pi^\star$. The standard regret decomposition (see \citet{dann2017unifying}, Lemma E.15) shows that the regret can be reformulated in terms of occupancy measures and sub-optimality gaps as  
\begin{equation}
\label{eq:regdef_gap}
Reg_T = \sum_{t=1}^T \sum_{s\in S\setminus \{s_L\},a\in A }q_t(s,a)\gap(s,a) = \sum_{t=1}^T\langle q_t,\gap\rangle .
\end{equation}
This decomposition further explains the sub-optimality gaps are analogous to the gap in stochastic multi-armed bandit  problem. 

\paragraph{Assumption on Uniqueness.} Throughout this paper, we assume the uniqueness of optimal policy. In other words, for every state $s$, $\gap(s,a) > 0$ if the action $a$ is not the optimal action $\pi^\star(s)$. We refer to \citet{zimmert2019optimal} for similar discussions on the uniqueness of the optimal bandit. It remains unclear whether we can drop this assumption in the this setting. 

On the other hand, in the \textit{adversarial} case $\ell_t$ is generated in an arbitrary way, in which it can depend on the learner's algorithm and randomness prior to episode $t$. 


